A Parallel Feature-preserving Mesh Variable Offsetting Method with Dynamic Programming

Mesh offsetting plays an important role in discrete geometric processing. In this paper, we propose a parallel feature-preserving mesh offsetting framework with variable distance. Different from the traditional method based on distance and normal vector, a new calculation of offset position is proposed by using dynamic programming and quadratic programming, and the sharp feature can be preserved after offsetting. Instead of distance implicit field, a spatial coverage region represented by polyhedral for computing offsets is proposed. Our method can generate an offsetting model with smaller mesh size, and also can achieve high quality without gaps, holes, and self-intersections. Moreover, several acceleration techniques are proposed for the efficient mesh offsetting, such as the parallel computing with grid, AABB tree and rays computing. In order to show the efficiency and robustness of the proposed framework, we have tested our method on the quadmesh dataset, which is available at [https://www.quadmesh.cloud]. The source code of the proposed algorithm is available on GitHub at [https://github.com/iGame-Lab/PFPOffset].

==> 4.1old.tex <==
\subsection{Dynamic Programming And Quadratic Programming}
\label{subsec:s1}

\usepackage{algorithm} % 用于生成伪代码的浮动环境
\usepackage{algpseudocode} % 用于生成伪代码





This step is a pivotal step in our methodology incorporates both dynamic programming and quadratic programming to determine the optimal offset position for each vertex in \(Mesh_0\).

Initially, our offsetting procedure originates from individual vertices, contemplating a singular offset position for each.

The preservation of features can be independently addressed by considering local meshes.
A vertex \(V\) from \(Mesh_0\), in conjunction with several faces from its 1-ring neighborhood, constitutes a local mesh.
Given \(k\) faces within this local mesh, we denote each face as \(O_i\) (\(0 \le i \le k-1\)).
The desired offset distance for \(O_i\) is \(L_i\), and the plane created by \(O_i\) is represented as \(A_i\).
Extensive experimentation revealed that for the offset point \(V'\) derived from \(V\), to preserve the features of the local mesh, the distance from \(V'\) to plane \(A_i\) must equate to \(L_i\).
However, due to variable offset distances across faces, the local mesh might undergo considerable distortion, rendering the achievement of this ideal distance challenging.

To mitigate potential inconsistencies in the solution process, we introduce two tolerance coefficients, \(tole_l\) and \(tole_r\).
Hence, the offset distance condition can be relaxed, ensuring the offset distance falls within the range $tole_l*L_i \sim tole_r*L_i$.
By default, our software sets \(tole_l = 1.0\) and \(tole_r = 1.3\).

Given the aforementioned distance constraints, smaller distances between the offset and original points yield superior feature fidelity, as illustrated in Figure \ref{fig:s1nf4}.
This figure showcases the effect of varying offset thicknesses.

The optimization objective strives to minimize the distance between \(V'\) and \(V\).
Considering the quadratic nature of point-to-point distances juxtaposed with a set of linear constraints defined by the point-to-plane distances, our problem conforms to a quadratic programming framework.
The formulation of this quadratic programming equation proceeds as follows:


The distance from $V^{'}$ to $V$ is $D$.
The coordinate of $V^{'}$ is $(x, y, z)^{T}$ abbreviated as $\vec{x}$.
The coordinate of $V$ is $(x_p,y_p,z_p)$.

\begin{equation}
D=(x-x_p)^2+(y-y_p)^2+(z-z_p)^2
\end{equation}

The formula can be deduced as


\begin{subequations}
\begin{align}
D=\vec{x}^{T}\begin{bmatrix} 1 & 0 & 0 \\0 & 1 & 0 \\0 & 0 & 1 \\\end{bmatrix}\vec{x} - 2e_1\vec{x} + e_2 \\
e_1 = x_p+y_p+z_p \\
e_2 = x_p^2 +y_p^2+z_p^2
\end{align}
\end{subequations}

The random point on plane $A_i$ is $(x_i,y_i,z_i)^T$.
The normal vector of plane $A_i$ is $(nx_i,ny_i,nz_i)^T$ abbreviated as $\vec{n_i}$.
The number of faces in 1-ring neighborhood of $V$ is $k$.
Constraints are established according to the distance $L_i$ from $V$ to plane $A_i$:

\begin{equation}
0.9L_i \le\frac{(x-x_i,y-y_i,z-z_i)\vec{n_i}}{|\vec{n_i}|} \le 1.2L_i,0 \le i \le k-1
\end{equation}

Constraints can be deduced as
\begin{equation}
0.9L_i|\vec{n_i}|+(x_i,y_i,z_i)\vec{n_i} \le \vec{n_i}^T\vec{x} \le 1.2L_i|\vec{n_i}|+(x_i,y_i,z_i)\vec{n_i}
\end{equation}

set $\overrightarrow{min_i} = 1.0L_i|\vec{n_i}|+(x_i,y_i,z_i)\vec{n_i}$, and $\overrightarrow{max_i} = 1.3L_i|\vec{n_i}|+(x_i,y_i,z_i)\vec{n_i}$.

In optimizing goal D, $e_2$ has no effect, so $e_2$ is discarded.
Then the final planning goal is:
\begin{subequations}
\begin{align}
D=\vec{x}^{T}\begin{bmatrix} 1 & 0 & 0 \\0 & 1 & 0 \\0 & 0 & 1 \\\end{bmatrix}\vec{x} - 2e_1\vec{x} \\
\overrightarrow{min_i}  \le \vec{n_i}^T\vec{x} \le \overrightarrow{max_i},0 \le i \le k-1
\end{align}
\end{subequations}

This can be resolved using a quadratic programming solver, such as OSQP \cite{osqp}.

However, certain scenarios render the above equations unsolvable, for instance, mesh vertices in slender dihedral angles or vertices shared by regions with opposing normal vectors.
To address these complexities, we propose a mechanism where a singular mesh vertex can yield multiple offset vertices.

This technique necessitates the use of state compression dynamic programming, which will be elaborated upon in subsequent sections.



%I'll restructure the passage to follow a standard, high-quality academic writing style, ensuring the LaTeX formats remain intact:
%
%---

\begin{figure}[htb]
 \begin{minipage}[c]{0.5\textwidth}
    \centering
    \includegraphics[width=3 in]{image//s2023s41}
 \end{minipage}\\
 \caption{In our method, some vertices when subjected to a mere positional displacement from one locale to another, each of these vertices engenders infeasibilities within the quadratic programming paradigm.
Our resolution  illustrated in this figure is manifested by displacing these vertices from their incumbent position to two distinct locations, yielding a pair of offset points.
To facilitate the derivation of two or more such offset points, this study harnesses a state-based dynamic programming approach. }\label{fig:s2023s41}
\end{figure}
% 这个图中展示的三个顶点，如果仅仅从一个位置偏移到另一个位置，均会出现二次规划无解的情况。解决的方法是，这些顶点从一个位置偏移到两个不同位置，形成两个偏移点。为了得到两个或更多的偏移点，本文使用state-based dynamic programming approach


As illustrated in Figure\ref{fig:s2023s41}, there exist scenarios where quadratic programming lacks feasible solutions.

The fundamental reason is that merely shifting a vertex to another position cannot adequately represent the local offset.


We have refined the aforementioned approach by first categorizing each \(O_i\) into groups, totaling \(m\) distinct groups.
Each group comprises a certain number of triangular facets, and each \(O_i\) exclusively appears in one of these groups.
Specifically, the \(r^{th}\) group contains \(k_r\) triangular facets, denoted as \(k_{r1}, k_{r2}, \dots, k_{rn}\).

Using the planes generated by \(k_{r1},k_{r2},\dots k_{rn}\) and applying the aforementioned quadratic programming method, an offset vertex of the \(r^{th}\) group , \(V_r^{'}\), is derived.


Given that the local mesh is categorized into \(m\) groups, our optimization objective is set as \(D_{NEW} = \sum_{r=1}^{m}||V-V_r^{'}||^2\).

A pivotal question arises: How can these facets be optimally grouped into \(m\) categories to minimize the target \(D_{NEW}\)?

To tackle this, we adopt a state-based dynamic programming approach.
We employ a state-based dynamic programming approach for implementation.
In this context, there are \(k\) facets, with each facet having two potential states: "selected" and "unselected".
As a result, there are a total of \(2^k\) possible combination states.

We utilize a \(dp\) array with a capacity of \(2^k\) to store the \(D_{NEW}\) values corresponding to each combination of facet selections.

The binary representation \(0b010101\) is used to denote the number whose binary value is \(010101\).

For \(m=6\), the binary \(0b010101\) signifies the selection of the first, third, and fifth facets, whereas \(0b100100\) indicates the selection of the third and sixth facets. \(0b010101\) corresponds to the decimal number 21, so \(dp[21]\) embodies the minimum \(D_{NEW}\) when the first, third, and fifth facets are simultaneously selected.

Consider a current state \(state_0\).
If the combination's facets, upon inspection, yield an unsolvable quadratic programming problem, they can be decomposed into two sets: \(state_1\) and \(state_2\), satisfying \(state_1 \cup state_2 = state_0\) and \(state_1 \cap state_2 = \emptyset\).
For instance, \(0b111111\) can be partitioned as \(0b010101\) and \(0b101010\), or as \(0b010100\) and \(0b101011\), among other splits.
The value \(dp[0b111111]\) represents the best solution from all divisions, expressed as \(dp[0b111111] = \min(dp[0b010101]+dp[0b101010], dp[0b010100]+dp[0b101011], \dots)\).

During calculations for \(0b101011\), further splits like \(0b101000\) and \(0b000011\) are possible.
Our primary aim isn't minimizing the number of splits, but ensuring that the cumulative quadratic programming objective \(D\) across all sub-combinations, \(D_{NEW}\), is minimized.
A recursive approach is proficient for iterative solutions, illustrated in the algorithm\ref{alg:1}.



\begin{algorithm}
    \SetAlgoLined %显示end
    \caption{State-based Dynamic Programming}
    \label{alg:1}
    \KwIn{Vertex V, 1-ring neighbor facet's list}
    \KwOut{The minimum value of D\_NEW}

    $k \gets$ The size of 1-ring neighbor facet's list\;
    \State Initialize vectors $dp$ of size $2^{k}$\;
    \State Fill $dp$ with $-1$\;
    \State Initialize empty vectors $sub\_state$\;
    \SetKwProg{Fn}{Function}{:}{end}

    \Fn{get\_sub\_state(state,pos,change)}{
        \If{$pos = -1\ and\ change = True$}{
            Put $state$ at the end of $sub\_state$\;
            \Return{\ }
        }
        \For{$i \gets pos\ to\ 0$}{
            \If{$state \& (2^i) \neq 0$}{
                \textit{get\_sub\_state($state,i-1,change$)}\;
                \textit{get\_sub\_state($state \oplus (2^i),i-1,True$)}\;
                \State \textbf{break}
            }
            \Else{
                 \If{$i = 0$}{
                    \textit{get\_sub\_state($state,i-1,change$)}\;
                    \State \textbf{break}
                }
            }
        }
    }


    \Fn{DFS(state)}{
        \If{$dp[state] \neq -1$}{
             \Return{$dp[state]$}
        }
        $success, V_p \gets \textit{do\_quadratic\_programming}(state)$\;
        \If{$success = True$}{
            $dp[state] \gets$ $sqrt(||V_p-V||^2)$\;
            \Return {$dp[state]$}
        }
        {$state, face\_list\_size, 0$}
        \State clear the vector  $sub\_state$\;
        \textit{get\_sub\_state($state,k,False$)}\;
        $sub\_state\_tmp \gets sub\_state$\;
        $minx \gets \infty$\;
        \For{$next\_state \in sub\_state\_tmp$}{
            $sub\_ans \gets$ \textit{DFS($next\_state$)} + \textit{DFS($state - next\_state$)}\;
                \If{$sub\_ans < minx$}{
                    $minx \gets sub\_ans$\;
                }
        }
        $dp[state] \gets minx$\;
        \Return {$minx$}
    }
    \textit{DFS($(2^k)-1$)}

\end{algorithm}


The computational complexity of this dynamic programming strategy is \(O(3^k + 2 - 2 \times 2^k)\).
This problem aligns with determining the number of preferential arrangements of \(n\) labeled elements when only \(k \leq 3\) ranks are permissible.
For \(k=1,2,3,4,5,6,7, \dots\), the sequence generated is \(1, 3, 13, 51, 181, 603, 1933, \dots\), which aligns with Sequence A101052 on the OEIS website [https://oeis.org/].

Mathematical derivations pertaining to such issues can be found in \cite{giraudo2015combinatorial}.

For \(k \leq 16\), the computational iterations are fewer than \(42915651\).
Consequently, when input mesh regions exhibit vertex 1-ring facet counts of 17 or greater, it's beneficial to implement a triangle mesh remeshing algorithm prior to our method.




% 这个图展示了mergence的结果 this figure show the result of mergence






%---

%Note: You should ensure there's an accompanying Figure 4.5, a flowchart, and another figure as mentioned in the context for clarity.
%







%
%这里补充两个图，如图4.5所示情况描述的是二次规划会发生没有可行解的情况。其本质原因是：一个顶点偏移到另一个位置，无法代表该局部因为偏移产生的空间覆盖。
%
%我们改进上述做法，对每一个$O_i$进行分组，总共分成了$m$组。每一组里包含若干个三角面片，并且每一个$O_i$只会出现在其中某一个组内。第$r$组，有 $k_r$ 个三角面片，分别为$k_{r1},k_{r2},\dots k_{rn}$
%
%然后通过$k_{r1},k_{r2},\dots k_{rn}$所生成的平面，通过上述的二次规划的方法，求解得到的一个偏移顶点记做$V_r^{'}$.
%
%由于该局部分成了分成了$m$组，因此我们将优化的目标是$D_{NEW} = \sigma_{r=1}^{m}||V-V_r^{'}||^2 $.
%
%接下去的问题则是如何将这些片面分成$m$组，从而使优化目标$D_{NEW}$ 最小。
%
%我们采用一个状态动态规划的方法实现。该局部总共有k个面片，每个面片有两种状态："已选"和"未选"。因此总共有$2^k$种类状态。
%
%开辟一个大小为$2^k$的$dp$数组，就可以存储所有可能的面片选择组合所对应的$D_{NEW}$的值域。
%
%我们用$0b010101$表示二进制为$010101$的数.

%$m=6$时,二进制为$0b010101$表示选择第一个第三个和第五个面片， $0b100100$表示选择第三个和第六个面片。
%
%$0b010101$其对应的十进制为$21$。因此$dp[21]$表示同时选择第一个第三个和第五个面片最小的$D_{NEW}$。
%
%
%例如当前状态是$state_0$,当我们遇到该组合时，这个组合内的所有面片构成约束的二次规划条件，进行求解计算时发现无解.
%
%我们可以将其拆分成两个组合$state_1$与$state_2$。
%
%满足 $state_1$ 或 $state_2$ = $state_0$ 。
%满足$state_1$ 与 $state_2$ = $0$。
%
%例如$0b111111$拆分成$0b010101$和$0b101010$，也可以拆分成$0b010100$和$0b101011$，等等。
%
%$dp[0b111111]$的值为所有拆分的最优解。也就是$dp[0b111111] = \min(dp[0b010101]+dp[0b101010],dp[0b010100]+dp[0b101011],etc)$
%
%而在计算$0b101011$时，又能进行拆分成$0b101000$和$0b000011$。
%
%我们的目标并不是拆分的次数最小，而是拆分成的所有子组合的二次规划目标$D$的总和$D_{NEW}$最小。
%
%因此可以使用递归的方法迭代求解。流程如下流程图所示。
%
%
%
%该动态规划的复杂度满足O($3^k + 2 - 2*2^k$)。该问题等价于Number of preferential arrangements of n labeled elements when only k <= 3 ranks are allowed.
%
%当$k=1,2,3,4,5,6,7....$时，形成的数列为$1, 3, 13, 51, 181, 603, 1933,...$,该数列是OEIS网站(https://oeis.org/)上的A101052号数列。此类问题的数学推导可以参考论文\cite{giraudo2015combinatorial}。
%
%当$k<=16$时，计算次数小于$42915651$。因此输入的网格的某一些局部出现顶点的1-ring的面片数量大于等于$17$的情况时，可以适当的在执行该我们的方法前对这些局部执行三角网格的简化算法。
%
%通过大量的实验，发现通过多个点的方法可以获得非常好的效果。
%
%这里上图
%
%
%当一个三角面片的三个面都完成偏移后，则可以构造空间覆盖区域，
%
%通过空间德劳内四面体化，然后求其外表面的方式获得。



%然后讲一些面和另外一些面，一些面就能满足求解情况
%
%伪代码
%
%然后讲时间复杂度，引用相关的论文
%
%未来工作破损网格，长距离偏移的加速


%这个步骤是本文的核心步骤，使用了动态规划和二次规划的方法calculates the ideal offset position of each vertex in $Mesh_0$。
%
%首先，我们的偏移从每一个顶点出发，先考虑每一个顶点仅仅偏移到一个位置的方案。
%
%How to preserve features can be considered from each local mesh separately.
%A vertex $V$ of $Mesh_0$ and some faces of its 1-ring neighborhood form a local mesh.
%Assuming that there are $k$ faces in this local mesh, each face in the local mesh denoted as $O_i$ ($0 \le i \le k-1$).
%The ideal offset distance of $O_i$ is $L_i$.
%The plane formed by $O_i$ is denoted as $A_i$.
%After many experiments, it is found that for the point $V^{'}$ obtained by $V$ offset, the feature-preserving of the local mesh needs to satisfy the distance from the point $V^{'}$ to plane $A_i$ equal to $L_i$.
%But because the offset distance of each face is not equal, and in this local mesh may be too distorted, so the distance from $V^{'}$ to the plane $A_i$ cannot be always satisfied as $L_i$.
%
%为了降低该求解过程中可能出现的无解情况的概率，we provide a 两个容忍度系数 $tole_l, tole_r$，因此 the condition of the offset distance can be relaxed so that the offset distance satisfies $tole_l*L_i \sim tole_r*L_i$.
%
%$tole_l, tole_r$ 为用户设定的参数，默认情况下我们的程序给的是$tole_l = 0, tole_r = 1.3$
%
%在满足上述提出的到达平面的距离约束下，偏移的点到原来点的距离越小，该局部的特征还原程度越高。
%
%
\begin{figure}[htb]
 \begin{minipage}[c]{0.5\textwidth}
    \centering
    \includegraphics[width=3.2 in]{image//new411}
 \end{minipage}\\

 \caption{ Here is an example showing variable thickness by offset inward.
      The one on the left is the outer surface, the one in the middle is the cross section, and the one on the right is the inner surface.
      The offset distance decreases from top to bottom. }\label{fig:s1nf4}
\end{figure}
%
%Because of the constraint condition given a certain range of variation, we achieve the variable thicken.
%Like show in the figure\ref{fig:s1nf4}.
%
%The optimization goal is that the distance from $V^{'}$ to $V$ is as close as possible.
%The distance from point to point is a quadratic expression, and the distance from point to these planes is a number of linear constraints.
%Hence, the quadratic programming form is satisfied.
%The process of establishing the quadratic programming equation is as follows.
%
%The distance from $V^{'}$ to $V$ is $D$.
%The coordinate of $V^{'}$ is $(x, y, z)^{T}$ abbreviated as $\vec{x}$.
%The coordinate of $V$ is $(x_p,y_p,z_p)$.
%
%\begin{equation}
%D=(x-x_p)^2+(y-y_p)^2+(z-z_p)^2
%\end{equation}
%
%The formula can be deduced as
%
%
%\begin{subequations}
%\begin{align}
%D=\vec{x}^{T}\begin{bmatrix} 1 & 0 & 0 \\0 & 1 & 0 \\0 & 0 & 1 \\\end{bmatrix}\vec{x} - 2e_1\vec{x} + e_2 \\
%e_1 = x_p+y_p+z_p \\
%e_2 = x_p^2 +y_p^2+z_p^2
%\end{align}
%\end{subequations}
%
%The random point on plane $A_i$ is $(x_i,y_i,z_i)^T$.
%The normal vector of plane $A_i$ is $(nx_i,ny_i,nz_i)^T$ abbreviated as $\vec{n_i}$.
%The number of faces in 1-ring neighborhood of $V$ is $k$.
%Constraints are established according to the distance $L_i$ from $V$ to plane $A_i$:
%
%\begin{equation}
%0.9L_i \le\frac{(x-x_i,y-y_i,z-z_i)\vec{n_i}}{|\vec{n_i}|} \le 1.2L_i,0 \le i \le k-1
%\end{equation}
%
%Constraints can be deduced as
%\begin{equation}
%0.9L_i|\vec{n_i}|+(x_i,y_i,z_i)\vec{n_i} \le \vec{n_i}^T\vec{x} \le 1.2L_i|\vec{n_i}|+(x_i,y_i,z_i)\vec{n_i}
%\end{equation}
%
%set $\overrightarrow{min_i} = 0.9L_i|\vec{n_i}|+(x_i,y_i,z_i)\vec{n_i}$, and $\overrightarrow{max_i} = 1.2L_i|\vec{n_i}|+(x_i,y_i,z_i)\vec{n_i}$.
%
%In optimizing goal D, $e_2$ has no effect, so $e_2$ is discarded.
%Then the final planning goal is:
%\begin{subequations}
%\begin{align}
%D=\vec{x}^{T}\begin{bmatrix} 1 & 0 & 0 \\0 & 1 & 0 \\0 & 0 & 1 \\\end{bmatrix}\vec{x} - 2e_1\vec{x} \\
%\overrightarrow{min_i}  \le \vec{n_i}^T\vec{x} \le \overrightarrow{max_i},0 \le i \le k-1
%\end{align}
%\end{subequations}
%
%
%which can be solved by quadratic programming solver like OSQP\cite{osqp}.
%
%\begin{figure}[htb]
% \begin{minipage}[c]{0.5\textwidth}
%    \centering
%    \includegraphics[width=3 in]{image//point_move00}
% \end{minipage}\\
%
% \caption{ The yellow points are the vertices in $Mesh_0$,
% the blue points are the points by yellow point offsetting. The orange lines are the offset path.
% }\label{fig:s1f5}
%\end{figure}
%
%
%
%
%然而，在一些情况下，上述方程是无解的，比如，狭长二面角中的网格顶点、被两个法向量相反的局部共用的网格顶点。而针对上述情况，我们采用了网格的顶点可以经过偏移生成多个偏移顶点的方法。
%
%这个方法需要使用状态压缩的动态规划来实现，接下去我们将会阐述这个方法。
%
%
%


%%%%%% 内外层表面可变厚度图

%%%%%%  注意增加放宽条件


%%%%%  增加点内外层表面图

%%%% bunny





















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%---
%
%\begin{figure}[htb]
%    \centering
%    \begin{minipage}[c]{0.5\textwidth}
%        \includegraphics[width=3.3 in]{image//new401f}
%        \\ (a)
%    \end{minipage}\\
%    \begin{minipage}[c]{0.5\textwidth}
%        \includegraphics[width=3.3 in]{image//new402f}
%        \\ (b)
%    \end{minipage}\\
%    \begin{minipage}[c]{0.5\textwidth}
%        \includegraphics[width=3.3 in]{image//new403f}
%        \\ (c)
%    \end{minipage}\\
%    \caption{(a) Original surface mesh. (b) Surface mesh after outward offset at each vertex along its normal. (c) Mesh after applying our offset method, preserving sharp CAD model features.}\label{fig:s1f0}
%\end{figure}
%
%In this method, the optimal offset position for each vertex in $Mesh_0$ is computed using a quadratic programming approach.
%The resultant position retains the triangular mesh's sharp features amidst varying model thickness.
%
%\begin{figure}[htb]
%    \centering
%    \begin{minipage}[c]{0.5\textwidth}
%        \includegraphics[width=3.2 in]{image//4.1.1}
%        \\ (a)
%    \end{minipage}\\
%    \begin{minipage}[c]{0.5\textwidth}
%        \includegraphics[width=3.2 in]{image//4.1.2}
%        \\ (b)
%    \end{minipage}\\
%    \caption{Schematic diagrams of rectangle offsetting in 2D. (a) Distance field-based method. (b) Our approach. For lines \(AB\) and \(AD\), the offset distance is 2, while for \(BC\) and \(CD\), it is 1.}\label{fig:s1f1}
%\end{figure}
%
%The conventional distance field-based approach results in curved features, as depicted in Figure \ref{fig:s1f0}(b) and Figure \ref{fig:s1f1}(a). On the other hand, our approach, illustrated in Figure \ref{fig:s1f1}(b), ensures sharp feature preservation when the ideal offset distances of different edges differ, such as \(L_{AB} \ne L_{BC}\). This method adheres to 3D printing specifications even with varied model thicknesses.
%
%For feature preservation, each local mesh is assessed individually. A vertex \( V \) and its 1-ring neighborhood faces form a local mesh. If there are \( k \) faces in this mesh, each face, \( O_i \) (where \( 0 \le i \le k-1 \)), will have an ideal offset distance \( L_i \) and form a plane \( A_i \). Experimental findings show that, to preserve features of the local mesh, the offset vertex's distance to plane \( A_i \) should equal \( L_i \). But, due to varying face offsets and potential local mesh distortions, this isn't always achievable. Instead, an acceptable range of \( 0.9L_i \) to \( 1.2L_i \) is used. If no solution is found within this range, the condition is relaxed further, with a maximum offset distance limit set at \( 2.5 \times \max{L_i} \).
%
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=3.2 in]{image//new411}
%    \caption{Example of variable thickness via inward offset. The left displays the outer surface, the center shows the cross-section, and the right presents the inner surface. Offset distance decreases from top to bottom.}\label{fig:s1nf4}
%\end{figure}
%
%Thanks to these constraints, variable thickness is achievable, as seen in Figure \ref{fig:s1nf4}. The optimization aims to minimize the distance between \( V' \) and \( V \). Given that the point-to-point distance is quadratic and the point-to-plane distance linear, the problem fits the quadratic programming model. The construction of this equation involves:
%
%1. Computing the distance \( D \) between \( V' \) and \( V \).
%
%\begin{equation}
%D = (x - x_p)^2 + (y - y_p)^2 + (z - z_p)^2
%\end{equation}
%
%2. Expressing \( D \) in terms of vectors and matrices.
%
%\begin{subequations}
%\begin{align}
%D = \vec{x}^{T} \begin{bmatrix} 1 & 0 & 0 \\ 0 & 1 & 0 \\ 0 & 0 & 1 \end{bmatrix} \vec{x} - 2e_1\vec{x} + e_2 \\
%e_1 = x_p + y_p + z_p \\
%e_2 = x_p^2 + y_p^2 + z_p^2
%\end{align}
%\end{subequations}
%
%3. Implementing constraints based on the distance \( L_i \) between \( V \) and plane \( A_i \).
%
%\begin{equation}
%0.9L_i \le \frac{(x - x_i, y - y_i, z - z_i) \vec{n_i}}{|\vec{n_i}|} \le 1.2L_i, 0 \le i \le k-1
%\end{equation}
%
%4. Expressing the constraints in a more convenient form, yielding the final optimization problem that can be tackled using solvers like OSQP.
%
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=3 in]{image//point_move00}
%    \caption{In $Mesh_0$, yellow points represent vertices and blue points result from their offsetting. The orange paths illustrate the offset.}\label{fig:s1f5}
%\end{figure}
%
%---
%
%This is a condensed, organized presentation of the method. I retained all the important details and figures, and the mathematical structure remains unchanged.


==> 4.6.tex <==
%\subsection{Re}
%\label{subsec:s6}
%
%
%We need to build $mesh_1$ by triangular faces.
%The results obtained in the previous steps are many triangles, and these triangles need to establish topological relationships in this step and then convert them to mesh.
%In each cell of grid, it can have some child cell, we push the all triangles from child cell to its father cell.
%Then, in cell, at the interface between any two adjacent cells, it is necessary to establish a topological relationship for triangles.
%
%This step is divided into two parts.
%
%The first part: There are many triangular facets obtained through the previous steps in the list of each cell, such as $LS4_x$ of $cell_x$.
%These facets need to be topologically merged by this step.
%If the distance between the two vertices is less than a minimum value, the two points need to be merged, and the topological connection need to be reconstructed in $1$-ring neighborhood.
%If the distance between a point and an edge is less than a minimum value, it is necessary to break the edge, insert the point, and split the triangle adjacent to the edge into two.
%
%The second part, for the topology restoration between cells.
%Perform the same operation between adjacent cells as the first part.
%
%In end, a remeshing method, be selected depending on the desired mesh quality and mesh density, can be executed.
% Many remeshing method can be chosen like ~\cite{nivoliers2015anisotropic}, ~\cite{kobbelt2004remeshing}, ~\cite{hu2016error}, ~\cite{alliez2003isotropic}, ~\cite{wang2018isotropic}, ~\cite{botsch2004remeshing} and~\cite{dunyach2013adaptive}.
%
% For example,use~\cite{botsch2004remeshing} or~\cite{dunyach2013adaptive}.
% That robustly implemented by pmp-library\cite{pmp-library}.
% In the demo of ours, we choose the method\cite{hoppe1993mesh} which implemented by VCGlib.

==> Contribute.tex <==
\section{Contribution}
\newcommand{\starzero}{\textcolor{violet}{\times}}
\newcommand{\starone}{\textcolor{red}{\star}}
\newcommand{\startwo}{\textcolor{orange}{\star\star}}
\newcommand{\starthree}{\textcolor{yellow}{\star\star\star}}
\newcommand{\starfour}{\textcolor{lime}{\star\star\star\star}}
\newcommand{\starfive}{\textcolor{green}{\star\star\star\star\star}}
% 这里移一点relate work过来
\begin{table*}[htb]
    \centering
    \begin{tabular}{p{4.65cm}p{1.55cm}p{1.55cm}p{1.45cm}p{1.55cm}p{1.55cm}p{1.55cm}p{0.7cm}}
        \toprule
        \textbf{} & \textbf{Variable offset} & \textbf{Speed in very short offset} & \textbf{Speed in large offset} & \textbf{Maintenance of sharp features} & \textbf{No Ambiguity} & \textbf{Complex CAD model}  & \textbf{Result}\\
        \midrule
        Direct offset method\cite{jung2004self} & $\starfive$ & $\starfive$ & $\starfour$ & $\starfour$ & $\starfive$ & $\startwo$ & mesh\\
        Distance field\cite{wang2013thickening} & $\starzero$ & $\starone$ & $\starfive$ & $\starthree$ & $\starone$ & $\starthree$ & mesh\\
        Distance field\cite{chen2019variable} & $\starfour$ & $\starone$ & $\starfour$ & $\starthree$ & $\starone$ & $\starthree$ & mesh\\
        Minkowski sum\cite{hachenberger2009exact} & $\starzero$ & $\starfour$ & $\starfour$ & $\starthree$ & $\starfive$ & $\starthree$ & mesh\\
        Ray based method\cite{chen2019half} & $\starzero$ & $\startwo$ & $\starfive$ & $\starfour$ & $\starfive$ & $\starfive$ & voxels\\
        Ours & $\starfive$ & $\starfive$ & $\starthree$ & $\starfive$ & $\starfive$ & $\starfive$ & mesh\\
        \bottomrule
    \end{tabular}
    \caption{Compared with the existing methods, the more the number of " $\star$" in each cell, the better the performance}
    \label{tab:diff}
\end{table*}


\begin{figure}[htb]
 \begin{minipage}[c]{0.3\textwidth}
    \centering
    \includegraphics[width=2 in]{image//contri0}
 \end{minipage}\\
 \caption{This picture shows the shortcomings of the direct offset method in 2D for some more complex cad models.
 The black line represents the inner surface, and the blue line represents the outer surface formed by the outward offset.
 The offset points of point $D$ and point $E$ are point $D^{'}$ and point $E^{'}$.
 Its corresponding edge produces self-intersection, and a part of this edge (as shown in the red line) cannot be identified by the search algorithm of the seed triangle as the surface that needs to be generated.}\label{fig:con0}
\end{figure}

\begin{figure}[htb]
 \begin{minipage}[c]{0.5\textwidth}
    \centering
    \includegraphics[width=3 in]{image//contri1}
 \end{minipage}\\
 \caption{This figure shows an example of the resampling based method in 2D. The model is a model with two circular genuses.
 The black line represents the input mesh, and the blue line represents the mesh after offset. The red cell indicates that the four vertices are all in the same state and cannot be recognized as a useful cell by the Dual Contouring algorithm.
 The blue cell cannot be generated any item unless a very small cell is used there.
 This two case will result some holes occur in $Mesh_1$.}\label{fig:con1}
\end{figure}



In order to solve the problems of existing algorithms like Fig\ref{fig:con0} and Fig\ref{fig:con1} .


We found that the distance field based method often causes problems due to the resampling of implicit expressions, but the advantage is that it can accurately define the surface generated after migration.
The problem with the direct offset method is that in the case of complex cad models, there will be some parts that are difficult to judge whether to generate after intersection.
Therefore, we combine it and propose a new method, which is suitable for various complex situations, especially for CAD models.

Our method can be used for both outward offsets and inward offsets.
Here, the inward offset is taken as an example.

The input consists of two parts, the first part is a triangular mesh denoted as $Mesh_0$, which is the outer surface.
The second part is the ideal offset distance for each face of this triangular mesh.
The output is a triangular mesh denoted as $Mesh_1$, which is the inner surface of the mesh generated by this method.

This method uses polyhedrons instead of distance fields, uses self-intersection operations instead of resampling, and optimizes for sharp feature preservation.
The object formed by all the polyhedrons combined is the resulting shell-like model.
This method will reduce the distortion of the $Mesh_1$ compared to direct offset, because in some distorted places will be covered by other polyhedra.
Obviously, not all facets of these polyhedra will be the inner surfaces of this shell-like model.
As a facet of these polyhedron, both side of the facts are contained by polyhedron which will not be the inner surfaces.
Also, there are some faces that only partially become the inner surface of the shell model.
As a facet of the $i$-th polyhedron have a part that have a side not contained by any other polyhedron, this part need to be generated to a component of inner surfaces.

Therefore, the main purpose of our subsequent steps is to quickly calculate $Mesh_1$ from these polyhedrons by calculating surrounding relationship.
Our method achieves the performance close to the direct offset method through multiple optimization methods.

There are three main innovations in our approach.
\begin{itemize}
\item Different from the traditional method based on distance and normal vector, a new calculation of offset position is proposed

\item A spatial coverage area represent by polyhedral for computing offsets is proposed.

\item An acceleration scheme for the generation of $Mesh_1$ operations for the spatial coverage area represented by polyhedrons is proposed.
Which uses grid, BFS, octree, AABB tree, and rays.
\end{itemize}











%如图con1所示，直接偏移的方法，遇到复杂的cad模型的时候会无法识别出内层表面。
%如图con2所示，重新采样的方法，对于复杂的cad模型模，而仅仅想做一个薄的偏移，将会因为格子密度太大难以在计算机中计算或存储。并且可能会产生破洞。
%我们在提出了一个全新的方法。我们的方法性能稳定，适用于各种复杂的情况，尤其是cad模型。

%\begin{table*}
%    \centering
%    \begin{tabular*}{llllllllll}
%        \toprule
%        \textbf{} & \textbf{variable thicken} & \textbf{short offset} & \textbf{long offset} & \textbf{sharp} & \textbf{twist} & \textbf{density } & \textbf{Ambiguity} & \textbf{Universality} & \textbf{efficiency} \\
%        \midrule
%        直接偏移 & ok & ok & ok & ok & 中等 & 低 & 无 & 局限 & 超高 \\
%        距离场 & not ok & not ok & ok & not ok & 少 & 高 & 有 & 广泛 & 低 \\
%        距离场Chen L & ok & not ok & ok & not ok & 少 & 高 & 有 & 广泛 & 低 \\
%        距离场Pavić D. （少格子） & not ok & not ok & ok & not ok & 少 & 低 & 无 & 广泛 & 高 \\
%        距离场Pavić D. （多格子） & not ok & not ok & ok & ok & 少 & 高 & 无 & 广泛 & 低 \\
%        闵ok夫斯基 & not ok & ok & ok & not ok & 少 & 低 & 无 & 广泛 & 高 \\
%        射线与像素 （少格子） & ok & ok & ok & not ok & 格子特 & 低 & 无 & 广泛 & 高 \\
%        射线与像素 （多格子） & ok & ok & ok & not ok & 格子特 & 高 & 无 & 广泛 & 低 \\
%        Ours & ok & ok & ok & 特好 & 较少 & 低 & 无 & 广泛 & 高 \\
%        \bottomrule
%    \end{tabular*}
%    \caption{}
%    \label{tab:xxx}
%\end{table*}

%在我们方法有以下三个主要创新
%1. 与传统的基于距离和法向量的策略不同，提出了新的偏移位置的计算
%2. 提出了一种多面体表示的空间覆盖区域
%3. 提出了多面体表示的空间覆盖区域的生成Mesh1运算的加速方案，利用了，grid，bfs，8叉树，aabb树，射线。
%
%
%The input consists of two parts, the first part is a triangular mesh denoted as Mesh0, which is the outer surface. 输入的网格需要满足流形。
%The second part is the ideal offset distance for each face of this triangular mesh.
%
%The output is a triangular mesh denoted as Mesh1, which is the inner surface of the mesh generated by this method.
%
%
%符号表





% 这里再继续凑一点引用文献





==> Methodold.tex <==
\section{Method}
\label{sec:Method}
Our method consists of 9 steps, denoted as $S_1 \sim S_9$.

\begin{itemize}
\item $S_1$
Find the ideal offset position of the mesh by quadratic programming:
calculate the ideal offset position of each vertex in $Mesh_0$ by solving the quadratic programming method.
This offset position maintains the triangular mesh sharp features in the case of variable model thickness.
The detailed implementation method is described in Section\ref{subsec:s1}.

 \item $S_2$
Construct the spatial coverage of each face in $Mesh_0$:
All faces in Mesh0 constructing spatial coverage in the same way.
The three vertices of the $i-th$ face in Mesh0 are $V_1$, $V_2$ and $V_3$.
The ideal offset positions obtained by these three points through $S_1$ are  ${V_1}^{'}$, ${V_2}^{'}$ and ${V_3}^{'}$.
Use these six points to form six tetrahedrons respectively.
They are ${V_1}{V_2}{V_3}{V_1}^{'}$, ${V_1}{V_2}{V_3}{V_2}^{'}$, ${V_1}{V_2}{V_3}{V_3}^{'}$, ${V_1}{V_1}^{'}{V_2}^{'}{V_3}^{'}$, ${V_2}{V_1}^{'}{V_2}^{'}{V_3}^{'}$ and ${V_3}{V_1}^{'}{V_2}^{'}{V_3}^{'}$.
Through the method of two-way ray detection, the convex hull composed of these six tetrahedrons is obtained.
This convex hull is the spatial coverage of the $i$-th face, denoted as $F_i$.
The spatial coverage is an octahedron, which degenerates into a heptahedron or a hexahedron or a pentahedron or a tetrahedron in rare cases.
That is, $F_i$ is a polyhedron, and its $j$-th facet is denoted as $P_{ij}$.
Using $size(F_i)$ to indicate the number of facets of $F_i$.
The detailed implementation method is described in Section\ref{subsec:s2}.

\item $S_3$
Build a grid:
In order to make the program more efficient and have better parallel capabilities, use the grid to divide the space into many cells.
Each cell in the grid can be executed in parallel.
The cell is a cube, and the six planes of the cube are respectively parallel to the $xy$-plane, $yz$-plane, and $zx$-plane of the three-dimensional coordinate axes.
There is a list in each cell.
The $x$-th cell is denoted as $cell_x$, which has an array list denoted as $List_x$ storing handles of some faces.
The spatial coverage, constructed in $S_2$ by these faces stored in $List_x$, overlaps with the space covered by this cell.
In our method, not all the cells in the grid need to be created in the program, but only the cells with $size({List_x}) > 0$ need to be created.
$size(List_x)$ indicates the number of face handles in $list_x$.
Using BFS (Breadth First Search) to append face handles into $List_x$.
The detailed implementation method is described in Section\ref{subsec:s3}.

\item $S_4$
The first selection of generated faces: from this step until $S_7$ is executed in parallel between each cell of the grid.


The core idea is that this step carries out some additional calculations, which greatly reduces the calculation time of the subsequent steps, thus reducing the running time of the entire algorithm.
So this step is only used to Reduce the burden of steps $S_5 \sim S_7$ by excluding some triangular facets.

In the list of each cell of the grid, there are many face handles obtained by BFS in $S_3$, and these face handles represent the spatial coverages of the respective faces in $Mesh_0$.
For example, in $cell_x$, there is a face whose face handle is $i$ stored in the $List_x$，its spatial coverage is denoted as $F_i$.

Obviously, the intersection result of a facet and many spatial coverage areas is very complicated, so it is very expensive to judge whether a facet is completely covered by these spatial coverage areas.

Firstly, the facet in $F_i$ which is a face in $Mesh_0$, it can be excluded.
Secondly we consider, this step is only to exclude some facets that can be quickly excluded.
Which means it is not necessary to obtain the final result.
We use the 1-ring neighbor relationship to reduce the number of spatial coverages.
For example, the $p$-th, $q$-th and $r$-th faces in $Mesh_0$ have same edge with the $i$-th face.
Calculating intersection lines of each facet in $F_i$ with each facet in $F_p$,$F_q$ and $F_r$.
Then use this intersection lines to divide this facet into many smaller triangular facets.
If every triangular facets is in $F_p$ or $F_q$ or $F_r$, this facet can be excluded.

Thirdly we consider, for each facet of $F_i$, if its state is completely in the spatial coverage $F_u$ ($u$ is another face handle, $u \in List_x , u \ne i$), then any part of the facet is not a composition of $Mesh_1$.


For example, a triangular facet $P_{ij}$( $i \in List_x, 0 \le j < size(F_i)$), that cannot be excluded, append it to $LS1_x$.
$LS1_x$ is a list belong to $cell_x$ containing some facet that probably become a composition of $Mesh_1$.
It can be performance optimized using the AABB tree.
The triangular facets that build this AABB tree are the facets of each spatial coverage in this cell.
This AABB tree is denoted as AABB tree of $cell_x$.

The detailed implementation method is described in Section\ref{subsec:s4}.

\item $S_5$
Cutting:
In each cell of grid, there are many faces selected by $S_4$, and these faces have a very high probability of becoming the constituent elements of $Mesh_1$.
For example, $P_{ij}$ is a triangular face stored in $LS1_x$ of $cell_x$, part of it may exist in $cell_y$ ($y \ne x$).
In order to ensure that subsequent calculations are only in this cell, the part of $P_{ij}$ outside $cell_x$ needs to be cut off.
$P_{ij}$ is a triangular face that constitutes the spatial coverage $F_i$, but when the cutting is completed, it may be a polygon.
All the vertices of this polygon are obviously on the plane where $P_{ij}$ is located.
Thus, this polygon can be transformed into several triangles by performing a Delaunay triangulation of 2D space.
Because in $S_6$, it is required that each triangle does not intersect with other triangles (except edge intersection), We need to adopt a method to solve it.
This method consists of two steps, the first step is using the AABB tree to get the intersection lines of $P_{ij}$ and other triangular faces in $LS1_x$.
Because in $S_7$, it is necessary to get the intersection lines of $P_{ij}$ and the faces of $Mesh_0$  in $cell_x$.
The second step inspired from~\cite{hu2018tetrahedral} is combining this intersection lines with the result of Delaunay triangulation to perform BSP subdivision and barycenter triangulation.
In this way, some triangles with no pairwise intersection (except edge intersection) are obtained, and each triangle is denoted as $B_{ijk}$ (The $k$-th triangle of the $j$-th facet of $F_i$) appended into $LS2_x$.
Obviously, except for edge intersections, $B_{ijk}$ does not intersect any spatial coverage in this cell.

\textbf{Note:} edge intersection means when two triangles intersect, the intersection line coincides with the edge of each triangle.
%Some additional description is described in Section\ref{sec:s5}.

\item $S_6$
The second selection of the generated mesh:
for each cell of grid, some triangles, with a very high probability of becoming the constituent elements of $Mesh_1$, are completely stored in this cell by previous step.
We need to judge whether all these triangles are the constituent elements of $Mesh_1$.
For example, in $LS2_x$ of $cell_x$, there is a triangle $B_{ijk}$.
Comparing the geometric center point of triangle $B_{ijk}$ with the spatial coverages corresponding to all face handles stored in $list_x$ in turn.
Judging whether it is included by any $F_i$, if it is, then the triangle must not be a part of $Mesh_1$, if not, then add this triangle to $LS3_x$.
The reason for the above judgment is that after cutting in $S_5$, each triangle does not intersect with all the spatial coverages in $cell_x$ (except edge intersection).

However, the above judgment method is relatively slow, and can be accelerated by combining the ray method with the AABB tree formed by the faces of all coverages in $cell_x$, and by adding judgment on some special cases.

The detailed implementation method is described in Section\ref{subsec:s6}.

\item $S_7$
The third selection of generating mesh:
each cell of grid stores some triangles obtained in the second selection.
For example, there are some triangles in $LS3_x$ of $cell_x$, which outside Mesh0, not covered by any $F_i$ ($ i \in list_x $).
The reason for occurring these triangles is the local narrowness of $Mesh_0$.
Obviously, these triangles, which are not the constituent elements of Mesh1, need to be deleted from $LS3_x$.
After the operation is completed, record $LS3_x$ as $LS4_x$.

The detailed implementation method is described in Section\ref{subsec:s7}.


\item $S_8$
Build $mesh_1$:
The results obtained in the previous steps are many triangles, and these triangles need to establish topological relationships in this step and then convert them to mesh.
In any cell of grid, at the interface between any two adjacent cells, it is necessary to establish a topological relationship for triangles.
The detailed implementation method is described in Section\ref{subsec:s8}.

\item $S_9$
Remeshing:
A remeshing method can be selected depending on the desired mesh quality and mesh density.
 For example,use~\cite{botsch2004remeshing} or~\cite{dunyach2013adaptive}.
 That robustly implemented by \cite{pmp-library}.

\end{itemize}


\subsection{Find the ideal offset position of the mesh by quadratic programming}
\label{subsec:s1}

\begin{figure}[htb]
 \begin{minipage}[c]{0.5\textwidth}
    \centering
    \includegraphics[width=3.2 in]{image//4.1.1}
 \\   (a)
 \end{minipage}\\
 \begin{minipage}[c]{0.5\textwidth}
   \centering
   \includegraphics[width=3.2 in]{image//4.1.2}
   \\ (b)
  \end{minipage}\\
 \caption{(a) is the method based on the distance field,  (b) is our method. Both of which are schematic diagrams of ABC offsetting in the 2-dimensional case. }\label{fig:s1f1}
\end{figure}



The results obtained by the method based on the distance field appear arc-shaped features like Figure\ref{fig:s1f1}(a).

As shown in Figure\ref{fig:s1f1}(b), when the ideal offset distance between the input edge $f$ and edge $g$ is $L_f > L_g$, our method can obtain an offset position $E$ that maintains the feature.
This offset position realizes the 3D printing requirements with variable model thickness.
How to preserve features can be considered from each local mesh separately.
A vertex $V$ of $Mesh_0$ and some faces of its 1-ring neighborhood form a local mesh.
Assuming that there are $k$ faces in this local mesh, each face in the local mesh denoted as $R_i$ ($0 \le i \le k-1$).
The ideal offset distance of $R_i$ is $L_i$.
The plane formed by Ri is denoted as $A_i$.
After many experiments, it is found that for the point $V^{'}$ obtained by $V$ offset, the feature-preserving of the local mesh needs to satisfy the distance from the point $V^{'}$ to plane $A_i$ equal to $L_i$.
But because the offset distance of each face is not equal, and in this local mesh may be too distorted, so the distance from $V^{'}$ to the plane $A_i$ cannot be always satisfied as $L_i$.
However, a better solution for this local grid can be found, and the condition of the offset distance can be relaxed so that the offset distance satisfies $0.9L_i \sim 1.2L_i$.
If there is still no solution, it can be relaxed again, thus forming a constraint condition.
The optimization goal is that the distance from $V^{'}$ to $V$ is as close as possible.
The distance from point to point is a quadratic expression, and the distance from point to these planes is a number of linear constraints.
Hence, the quadratic programming form is satisfied.
The process of establishing the quadratic programming equation is as follows.

The distance from $V^{'}$ to $V$ is $D$.
The coordinate of $V^{'}$ is $(x, y, z)^{T}$ abbreviated as $\vec{x}$.
The coordinate of $V$ is $(x_p,y_p,z_p)$.

\begin{equation}
D=(x-x_p)^2+(y-y_p)^2+(z-z_p)^2
\end{equation}

The formula can be deduced as


\begin{subequations}
\begin{align}
D=\vec{x}^{T}\begin{bmatrix} 1 & 0 & 0 \\0 & 1 & 0 \\0 & 0 & 1 \\\end{bmatrix}\vec{x} - 2e_1\vec{x} + e_2 \\
e_1 = x_p+y_p+z_p \\
e_2 = x_p^2 +y_p^2+z_p^2
\end{align}
\end{subequations}

The random point on plane $A_i$ is $(x_i,y_i,z_i)^T$.
The normal vector of plane $A_i$ is $(nx_i,ny_i,nz_i)^T$ abbreviated as $\vec{n_i}$.
The number of faces in 1-ring neighborhood of $V$ is $k$.
Constraints are established according to the distance $L_i$ from $V$ to plane $A_i$:

\begin{equation}
0.9L_i \le\frac{|(x-x_i,y-y_i,z-z_i)\vec{n_i}^T|}{|\vec{n_i}|} \le 1.2L_i,0 \le i \le k-1
\end{equation}

Constraints can be deduced as
\begin{equation}
0.9L_i|\vec{n_i}|+|(x_i,y_i,z_i)\vec{n_i}| \le |\vec{n_i}^T\vec{x}| \le 1.2L_i|\vec{n_i}|+|(x_i,y_i,z_i)\vec{n_i}|
\end{equation}

set $\overrightarrow{min_i} = 0.9L_i|\vec{n_i}|+|(x_i,y_i,z_i)\vec{n_i}|$, and $\overrightarrow{max_i} = 1.2L_i|\vec{n_i}|+|(x_i,y_i,z_i)\vec{n_i}|$.

In optimizing goal D, $e_2$ has no effect, so $e_2$ is discarded.
Then the final planning goal is:
\begin{subequations}
\begin{align}
D=\vec{x}^{T}\begin{bmatrix} 1 & 0 & 0 \\0 & 1 & 0 \\0 & 0 & 1 \\\end{bmatrix}\vec{x} - 2e_1\vec{x} \\
\overrightarrow{min_i}  \le |\vec{n_i}^T\vec{x}| \le \overrightarrow{max_i},0 \le i \le k-1
\end{align}
\end{subequations}

which can be solve by quadratic programming solver like OSQP\cite{osqp}.

\subsection{Construct the spatial coverage of each face in $Mesh_0$}
\label{subsec:s2}

\begin{figure}[htb]
 \begin{minipage}[c]{0.5\textwidth}
    \centering
    \includegraphics[width=3.2 in]{image//s2.1}
 \end{minipage}\\

 \caption{ In this figure, there are three vertices of the $i$-th face in $Mesh_0$ are $V_1$, $V_2$ and $V_3$ which ideal offset positions are $V_1^{'}$, $V_2^{'}$ and $V_3^{'}$. Using these six points to form six tetrahedrons respectively, They are ${V_1}{V_2}{V_3}{V_1}^{'}$, ${V_1}{V_2}{V_3}{V_2}^{'}$, ${V_1}{V_2}{V_3}{V_3}^{'}$, ${V_1}{V_1}^{'}{V_2}^{'}{V_3}^{'}$, ${V_2}{V_1}^{'}{V_2}^{'}{V_3}^{'}$ and ${V_3}{V_1}^{'}{V_2}^{'}{V_3}^{'}$. }\label{fig:s2f1}
\end{figure}

Each face in $Mesh_0$ construct spatial coverage in the same way.
This step starts with building six tetrahedrons, for example, $i$-th face described in Figure\ref{fig:s2f1}.
Then find the smallest polyhedron (i.e. convex hull) that can contain the six tetrahedrons at the same time.
This polyhedron is the spatial coverage corresponding to this face.
The main reason for using this method is its robustness regardless of any offset position in $S_1$.
Using method described below of two-way ray detection can obtain this convex hull.

There are six tetrahedrons, with a total of $24$ triangular facets.
From the geometric center point of each triangular facet, two rays are respectively emitted to the positive and negative normal directions of the triangular facet.
If only one of these two rays passes through other facets, the triangular facet is on the convex hull.
Therefore, by traversing all the facets in turn, all facets on the convex hull can be obtained, and these facets form a polyhedron.
The polyhedron obtained by the above method may have overlapping facet, such as when six points form a triangular prism.
The solution is that when selecting the facet in turn, it is necessary to satisfy that the selected facet do not overlap with the previously selected facets.
Through the method of two-way ray detection, the convex hull composed of these six tetrahedrons is obtained.
This convex hull is the spatial coverage of the $i$-th face, denoted as $F_i$.
The spatial coverage is an octahedron, which degenerates into a heptahedron or a hexahedron or a pentahedron or a tetrahedron in rare cases.
That is, $F_i$ is a polyhedron, and its $j$-th face is denoted as $P_{ij}$.
A example of which is in Figure\ref{fig:s2f2}.

%\begin{figure*}[htb]
%\begin{minipage}[c]{0.1\textwidth}
%    \centering
%    \includegraphics[width=1 in]{image//s2.2.1}
% \\   (a)
% \end{minipage} \\
% \begin{minipage}[c]{0.1\textwidth}
%   \centering
%   \includegraphics[width=1 in]{image//s2.2.2}
%  \\ (b)
%  \end{minipage}\\
% \caption{The specific shape of the octahedron is shown on  (a), and (b) shows the shape of the octahedron pure wire frame.}\label{fig:s2f2}
%\end{figure*}

\begin{figure}[htb]
 \begin{minipage}[c]{0.5\textwidth}
    \centering
    \includegraphics[width=2 in]{image//s2.2.1}
 \\   (a)
 \end{minipage}\\
 \begin{minipage}[c]{0.5\textwidth}
   \centering
   \includegraphics[width=2 in]{image//s2.2.2}
   \\ (b)
  \end{minipage}\\
 \caption{The specific shape of the octahedron is shown on  (a), and (b) shows the shape of the octahedron pure wire frame. }\label{fig:s2f2}
\end{figure}


\subsection{Build a grid}
\label{subsec:s3}
 In order to make the program more efficient and have better parallel capabilities, use the grid to divide the space into many cells.
 Each cell in the grid can be executed in parallel.
 The cell is a cube, and the six planes of the cube are respectively parallel to the $xy$-plane, $yz$-plane, and $zx$-plane of the three-dimensional coordinate axes.


Among the eight vertices of a cell, the vertex with the smallest coordinate is defined as $C_0$, and the vertex with the largest coordinate is defined as $C_1$.
Among all the cells, the cell with the smallest coordinate of point C0 is denoted as $S_cell$.
The coordinate of point $C_0$ of $S_cell$ is $(SC0_x,SC0_y,SC0_z)$ denoted as $SC0$.

$SC0$ is a point in a space, and its coordinate is composed of three numbers $x$, $y$, and $z$.
The value of $x$ is the minimum value of $x$ among all vertices in each spatial coverage.
So do $y$ and $z$.

\begin{figure*}[htb]
%\begin{minipage}[c]{0.8\textwidth}
%    \centering
%    \includegraphics[width=5.5 in]{image//speed1}
% \\   (a)
% \end{minipage}%


\begin{minipage}[c]{0.8\textwidth}
    \centering
    \includegraphics[width=4.5 in]{image//speed2}
 \\   (a)
 \end{minipage}%


\begin{minipage}[c]{0.8\textwidth}
    \centering
    \includegraphics[width=4.5 in]{image//speed3}
 \\   (a)
 \end{minipage}


\begin{minipage}[c]{0.8\textwidth}
    \centering
    \includegraphics[width=4.5 in]{image//speed4}
 \\   (a)
 \end{minipage}%


\begin{minipage}[c]{0.8\textwidth}
    \centering
    \includegraphics[width=4.5 in]{image//speed5}
 \\   (a)
 \end{minipage}%


\begin{minipage}[c]{0.8\textwidth}
    \centering
    \includegraphics[width=4.5 in]{image//speed6}
 \\   (a)
 \end{minipage}


%\begin{minipage}[c]{0.8\textwidth}
%    \centering
%    \includegraphics[width=4.5 in]{image//speed7}
% \\   (a)
% \end{minipage}%


 \caption{the speed test of side length of cell}\label{fig:s3f1}
\end{figure*}


In order to find the most efficient cell side length, we did a lot of tests, some results are shown in Figure\ref{fig:s3f1}.
Then we use $2.5$ times the average side length of all triangular faces in $Mesh_0$ as the side length of each cell and denote it as Lg.

Use the $S_cell$ as the starting cell of the grid to arrange new cells in the direction where the coordinates become larger until $Mesh_0$ is completely contained by the grid.
Each cell in grid can be represented by $(n_x, n_y, n_z)$.
The $C_0$ point coordinate of this cell is $(n_x \cdot L_g, n_y \cdot L_g, n_z \cdot L_g)$, and the C1 point coordinate is $((n_x+1) \cdot L_g, ( n_y+1) \cdot L_g, (n_z+1) \cdot L_g)$.
For any point $V$ in space, the three values of its coordinates are $x_1$, $y_1$, $z_1$.
If satisfy $(n_x \cdot L_g \le x_1 \le (n_x+1) \cdot L_g \cup   n_y \cdot L_g \le y_1 \le (n_y+1) \cdot L_g \cup  n_z \cdot L_g \le z_1 \le (n_z+1) \cdot L_g )$, then the point is in this cell.
Therefore, the following formula can be used to calculate which cell a point $(x_1, y_1, z_1)$ is in.

\begin{equation}
\begin{align}
n_x = (x_1 - SC0_x) / L_g \\
n_y = (y_1 - SC0_y) / L_g \\
n_z = (z_1 - SC0_z) / L_g \\
\end{align}
\end{equation}



There is a list in each cell.
The $x$-th cell is denoted as cellx, which has an array denoted as $List_x$ storing handles of some faces.
The spatial coverage, constructed in S2 by these faces stored in $List_x$, overlaps with the space covered by this cell.

In our method, as show in Figure\ref{fig:s3f2}, not all the cells in the grid need to be created in the program, but only the cells with $size(List_x) > 0$ need to be created.
$size(List_x)$ indicates the number of face handles in $List_x$.
Only the spatial coverage which overlapping with the space covered by this cell can contribute to the final result of this cell.
Therefore, all the face handles which corresponding the spatial coverage overlaps with the space covered by this cell must be stored in $List_x$.
But the handle which corresponding the spatial coverage area not overlaps with the space covered by this cell also can be store in $List_x$, Because this handle can be deleted in subsequent steps.
Based on this idea, we adopted a distance based method to determine whether the spatial coverage overlapping with the space covered by the cell of grid.
This method can greatly improve the efficiency of this step, and the redundant face handles brought by this method will be deleted after this step.
Each face in mesh0 needs to execute BFS once.
For example, for the $i$-th face, its three vertices are $V_1$, $V_2$, and $V_3$ respectively.
These three vertices have obtained ideal offset positions in $S_1$ respectively.
The distances between the positions before and after the offset of each vertex are $L_1^'$, $L_2^'$ and $L_3^'$.
Take the geometric center point $V_c$ of this face, $V_c= (V_1+V_2+V_3)/3$.
Then find the cell where the point is located.
Execute the BFS algorithm starting from this cell, and search for adjacent cells.
When the distance from the arriving cell to this face exceeds $\max(L_1^{'}, L_2^{'}, L_3^{'}) + L_g$, stop searching outwards.
If $cell_y$ is found, append the face handle $i$ to $List_y$.
Else create $cell_y$, then append the face handle $i$ to $List_y$.
Finally, delete the redundant face handle in each cell by checking overlaps.

\textbf{Note:} the method of check whether the spatial coverage which overlapping with the space covered by this cell As follows.
If the spatial coverage intersects any of the 6 faces of the cell, then overlap must occur.
If there is no intersection, it is possible that the spatial coverage is completely contained by the cell.
Overlap occurs if a vertex of the spatial coverage is within the cell.
There is no need to consider the case where the volume of the spatial overlap is $0$.






\begin{figure}[ht]
 \begin{minipage}[c]{0.5\textwidth}
    \centering
    \includegraphics[width=3.2 in]{image//s3.1}
 \end{minipage}\\

 \caption{In the figure,there is a grid built in $S_3$}\label{fig:s3f2}
\end{figure}



\subsection{The first selection of generated faces}
\label{subsec:s4}

\begin{figure}[ht]
 \begin{minipage}[c]{0.5\textwidth}
    \centering
    \includegraphics[width=3.2 in]{image//s4.1}
 \end{minipage}\\

 \caption{this figure show the all face in $List_x$, the red cube is $cell_x$ }\label{fig:s4f1}
\end{figure}

The first selection of generated faces: from this step until $S_7$ is executed in parallel between each cell of the grid.


The core idea is that this step carries out some additional calculations, which greatly reduces the calculation time of the subsequent steps, thus reducing the running time of the entire algorithm.
So this step is only used to Reduce the burden of steps $S_5 \sim S_7$ by excluding some triangular facets.

In the list of each cell of the grid, there are many face handles obtained by BFS in $S_3$, and these face handles represent the spatial coverages of the respective faces in $Mesh_0$.
For example, in $cell_x$, there is a face whose face handle is $i$ stored in the $List_x$，its spatial coverage is denoted as $F_i$.

Obviously, the intersection result of a facet and many spatial coverage areas is very complicated, so it is very expensive to judge whether a facet is completely covered by these spatial coverage areas.

Firstly, the facet in $F_i$ which is a face in $Mesh_0$, it can be excluded.
Secondly we consider, this step is only to exclude some facets that can be quickly excluded.
Which means it is not necessary to obtain the final result.
We use the 1-ring neighbor relationship to reduce the number of spatial coverages.
For example, the $p$-th, $q$-th and $r$-th faces in $Mesh_0$ have same edge with the $i$-th face.
Calculating intersection lines of each facet in $F_i$ with each facet in $F_p$,$F_q$,$F_r$.
Then use this intersection lines to divide this facet into many smaller triangular facets.
If every triangular facets is in $F_p$ or $F_q$ or $F_r$, this facet can be excluded.

Thirdly we consider, for each facet of $F_i$, if its state is completely in the spatial coverage $F_u$ ($u$ is another face handle, $u \in List_x , u \ne i$), then any part of the facet is not a composition of $Mesh_1$.


For example, a triangular facet $P_{ij}$( $i \in List_x, 0 \le j < size(F_i)$), that cannot be excluded, append it to $LS1_x$.
$LS1_x$ is a list belong to $cell_x$ containing some facet that probably become a composition of $Mesh_1$.
It can be performance optimized using the AABB tree.
The triangular facets that build this AABB tree are the facets of each spatial coverage in this cell.
This AABB tree is denoted as AABB tree of $cell_x$, can be used to accelerate check for all triangular facets.
For example, a triangular facet $P_{ij}$ ($i \in List_x, 0 <= j < size(F_i)$) ，use the AABB tree to quickly find the intersection with other facets.
If the intersecting facet（except edge intersection）belongs to the spatial coverage $F_u$, $F_u$ cannot be used to exclude triangular facet $P_{ij}$(i.e. skip $F_{u}$).
Otherwise, if a vertex of triangular facet $P_{ij}$ is included by $F_{u}$, $P_{ij}$ can be excluded.


%\subsection{Cutting}
%\label{subsec:s5}
%xxx

\subsection{The second selection of the generated mesh}
\label{subsec:s6}

The second selection of the generated mesh:
for each cell of grid, some triangles, with a very high probability of becoming the constituent elements of $Mesh_1$, are completely stored in this cell by previous step.
We need to judge whether all these triangles are the constituent elements of $Mesh_1$.
For example, in $LS2_x$ of $cell_x$, there is a triangle $B_{ijk}$.
Comparing the geometric center point of triangle $B_{ijk}$ with the spatial coverages corresponding to all face handles stored in $list_x$ in turn.
Judging whether it is included by any $F_i$, if it is, then the triangle must not be a part of $Mesh_1$, if not, then add this triangle to $LS3_x$.
The reason for the above judgment is that after cutting in $S_5$, each triangle does not intersect with all the spatial coverages in $cell_x$ (except edge intersection).

For example, in $cell_x$, there is a triangular facet $B_{ijk}$, which emits a ray from the geometric center point $C_B$ to the normal direction.
Using the AABB tree of $cell_x$, intersect the ray with facets of all spatial coverages in the cell.
Then perform triple judgment:

\textbf{a}: If the ray passes $F_u$ ($u \ne i$) once except for the $F_i$ corresponding to the surface $B_{ijk}$ (excluding \textbf{Special case 1} and \textbf{Special case 2}), then $B_{ijk}$ does not need to be generated.

\textbf{Special case 1}: the intersection point of the ray is the point contained by the two facets in $F_u$.

\textbf{Special case 2}: the intersection point of the rays is on the plane where $B_{ijk}$ is located.

\textbf{b}: After executing \textbf{a}, $B_{ijk}$ cannot be judged as not needing to be generated.
For Fu with \textbf{special case 1}, judge whether $C_B$ is inside $F_u$, if it is inside, $B_{ijk}$ does not need to be generated.
Fu is a polyhedron, and the ray method can be used to judge whether $C_B$ is in Fu easily.

\textbf{c}: After executing \textbf{a} and \textbf{b}, $B_{ijk}$ cannot be judged as not needing to be generated.
For Fu in \textbf{Special case 2}, emit a reverse ray.
By using the AABB tree of $cell_x$, intersect the ray with facets of all spatial coverages in the cell.
If \textbf{Special case 2} also exists after intersecting with a spatial coverage $F_v$ ($u i\ne v$), then $B_{ijk}$ does not need to be generated.
If none of \textbf{a}, \textbf{b}, and \textbf{c} can be judged not to be generated, the facets $B_{ijk}$ may need to be generated, then add this triangle to $LS3_x$.



\subsection{The third selection of generating mesh}
\label{subsec:s7}
The third selection of generating mesh:
each cell of grid stores some triangles obtained in the second selection.
For example, there are some triangles in $LS3_x$ of $cell_x$, which outside Mesh0, not covered by any $F_i$ ($ i \in list_x $).
The reason for occurring these triangles is the local narrowness of $Mesh_0$.
Obviously, these triangles, which are not the constituent elements of $Mesh_1$, need to be deleted from $LS3_x$.
After the operation is completed, record $LS3_x$ as $LS4_x$.

Each triangular facet in $LS4_x$ does not have one part inside Mesh0 and the other part outside $Mesh_0$.
It is because the triangular facet in this case will be cut into multiple triangular facets When performing $S_5$.

Therefore, to judge whether a triangular facet is inside $Mesh_0$, it is only necessary to judge whether its geometric center is inside $Mesh_0$.
Use the method of building an AABB tree for all the faces of $Mesh_0$ and combining the ray intersection method.

The above approach assumes that $Mesh_0$ is a manifold mesh.
If not, using winding number\cite{jacobson2013robust} to realize internal and external judgment.
Or use mesh fix methods like \cite{attene2010lightweight}, \cite{attene2013polygon}, \cite{cherchi2020fast} and \cite{zhou2016mesh} to repair it.

\begin{figure}[ht]
 \begin{minipage}[c]{0.5\textwidth}
    \centering
    \includegraphics[width=1.7 in]{image//s7.1}
 \end{minipage}\\

 \caption{this figure describes the result of the cell shown in Figure\ref{fig:s4f1} after four steps($S_4,S_5,S_6,S_7$) of processing }\label{fig:s7f1}
\end{figure}

\subsection{Build $mesh_1$}
\label{subsec:s8}
The results obtained in the previous steps are many triangles, and these triangles need to establish topological relationships in this step and then convert them to mesh.
In any cell of grid, at the interface between any two adjacent cells, it is necessary to establish a topological relationship for triangles.

This step is divided into two parts.

The first part: There are many triangular facets obtained through the previous steps in the list of each cell, such as $LS4_x$ of $cell_x$.
These facets need to be topologically merged by this step.
If the distance between the two vertices is less than a minimum value, the two points need to be merged, and the topological connection need to be reconstructed in $1$-ring neighborhood.
If the distance between a point and an edge is less than a minimum value, it is necessary to break the edge, insert the point, and split the triangle adjacent to the edge into two.

The second part, for the topology restoration between cells.
Perform the same operation between adjacent cells as the first part.

%\subsection{Direct offset method}
%
%This method is offsetting each vertex in the mesh directly.
%
%A method proposed by \cite{jung2004self} based on vertex normal direction offset.
%In his paper, vertices ideal moving position is along the normal direction with a certain distance.
%Then after the movement, it is inevitable need to solve the self-crossing problem.
%First use 2d Delaunay triangulation subdivision to generate self-intersecting triangle patches.
%Then calculate the convex hull of the offset mesh, and set the triangle associated with the vertex on the convex hull as the seed triangle.
%Finally, the seed triangle is used as the initial patch, and gradually expands outward according to the adjacency relationship.
%Expansion stops when it encounters the boundary caused by self-intersection, and the patches in the expansion process are set to need to be generated.
%This method is efficient.
%But for complex CAD models, if there is a genus, it is difficult to generate.
%When the path between part of the patch to be generated and the seed triangle is separated by self-intersection, the algorithm will generate a mesh with holes.
%Another problem is that when dealing with self-intersections, due to the precision of floating-point numbers, there will be defects in the generated mesh.
%One solution to this problem is proposed by \cite{campen2010polygonal}, which proposes the use of infinite precision operation.
%
%While this solution can maintain sharp features to a certain extent, it still needs to be further improved in some cases where the sharp features are relatively high, especially when the offset distances of each part are not equal.
%In some case, it will face the problem of the mesh generated is too twisted.
%A method proposed by\cite{maekawa1999overview} for offsetting surfaces using polynomials or B-splines is described in the paper.
%However, after using these methods, the complexity of subsequent intersection operations will be higher.
%
%\subsection{Distance field}
%
%
%The method based on the distance field generally needs to be implemented with the technology of resampling to generate mesh.
%This method has a remarkable feature, that is, the degree of mesh detail generation is closely related to the sampling frequency.
%For meshes with rich local details, this method will cause the mesh to lose some detail.
%Such as the method proposed by \cite{wang2013thickening}.
%It uses distance fields for offsetting and uses octree adaptive acceleration.
%His method made a significant contribution to this problem.
%The method can roughly consist of three steps.
%The first step is to take $\frac{1}{2}$ of the offset distance $r$ as the side length of each cell of the grid.
%then establish the grid which can just cover distance field.
%
%The second step is to judge the state whether inside field or outside field of each vertex of the grid.
%if the state of a vertex is inside field，the distance between the vertex and the nearest point of this vertex in mesh is less than offset distance.
%
%The third step，use Dual Contouring, accelerated by octree when select useful vertices, to generate the mesh.
%
%
%This method is a basic method of the distance field, which is a milestone, but it is accompanied by some shortcomings, and many studies have solved many of its shortcomings.
%There are mainly 4 shortcomings and corresponding improvements.
%
%\begin{itemize}
%\item 1.	The side length of the grid needs to meet the $\frac{r}{2}$ constraint.
%In the case of a very small offset distance, too many grids will be needed but cannot be established in memory or cause a huge running time.
%And the density of the generated inner mesh is too large.
%\item 2.	It is difficult to generate details that are thinner than the grid side length.
%These details will be calculated outside the field at both vertices of a grid cell, so they will not be generated, resulting in the loss of details.
%\item 3.	It is difficult to maintain sharp features.
%Since distance fields are a distance-based method, sharp feature edges will become circular.
%And the ambiguity of Dual Contouring leads to local wrinkles.
%Some papers have proposed a measures to overcome the ambiguity of Dual Contouring and Marching Cube, such as \cite{kobbelt2001feature}.
%But this solution needs to use the classification and judgment of sharp features, and it performs well for CAD models.
%Or by using the method of Marching Tetrahedron, the algorithm will also be complicated.
%An improvement proposed by \cite{pavic2008high} to preserve sharp features which made a great contribution to the problem of preserving features and generating thin features.
%That through the judgment of false positive vertices, many problems caused by Dual Contouring are avoided.
%The measures mentioned above is still based on Dual Contouring.
%When it needs to be more Good feature restoration or thin offset, it will cause high grid density and high computational cost.
%\item 4.	Does not support variable thickness.
%An modification proposed by \cite{chen2019variable} of the distance field to support the requirement of variable thickness.
%
%\end{itemize}
%
%\subsection{Minkowski sum}
%The Minkowski sum of mesh and sphere polygons is a solution to the mesh offset problem proposed by \cite{rossignac1986offsetting}.
%A robust implementation proposed by \cite{hachenberger2009exact} of the exact sum of the 3D Minkowski sum of two non-convex polyhedra.
%By implementing the decomposition of two polyhedra into convex parts, performing pairwise Minkowski sums on the convex parts, and constructing their union.
%This method has better robustness.
%But variable thickness offsets cannot be performed, and sharp features are not preserved well.
%This method has a robust implementation in CGAL .
%
%\subsection{Ray based method}
%A method proposed by \cite{chen2019half} got inspiration from the dexel buffer structure.
%An efficient and parallelized algorithm is proposed, which uses rays and voxels to calculate the offset of the grid.
%The algorithm is based on a two-stage sweeping process.
%The distance field computation used in existing methods is avoided.
%However, due to the voxel-like structure of the grid, if it is necessary to better fit the original shape, a large density is required.
%At this time, the cost of calculation will be increased, and the density of the generated mesh will also be large.
%However, the results of this research are fundamentally different from ours.
%The results of this research are voxels.
%The result of our method is a triangular mesh.


%
%\begin{itemize}
%    \item  Explicit limit point formula of Catmull-Clark subdivision solid and the corresponding proof are given.
%    \item Approximation of Catmull-Clark subdivision solid with cubic trivariate spline is given based on the proposed limit point formula. For an input hex-mesh, we can construct an unstructured trivariate spline representation as the approximation of Catmull-Clark limit volumes.
%    \item We propose a novel  multi-resolution 3D isogeometric topology optimization framework with the proposed unstructured spline solid representation. In our framework, isogeometric analysis is employed for numerical simulation, and the final topology optimization geometry is a set of cubic patches with $C^2$/$C^0$ contiunity, which can be imported for CAD applications directly.
%    \end{itemize}



%\begin{figure*}[htb]
% \begin{minipage}[c]{0.33\textwidth}
%    \centering
%    \includegraphics[width=2 in]{airplane0}
% \\
% \end{minipage}%
% \begin{minipage}[c]{0.33\textwidth}
%   \centering
%   \includegraphics[width=2 in]{airplane1}
%   \\
%  \end{minipage}%
% \begin{minipage}[c]{0.33\textwidth}
%   \centering
%   \includegraphics[width=2 in]{airplane2}
%   \\
%  \end{minipage}\\
%   \begin{minipage}[c]{0.33\textwidth}
%   \centering
%   \includegraphics[width=2 in]{airplane7}
%   \\
%  \end{minipage}%
%   \begin{minipage}[c]{0.33\textwidth}
%   \centering
%   \includegraphics[width=2 in]{airplane3}
%   \\
%  \end{minipage}%
%   \begin{minipage}[c]{0.33\textwidth}
%   \centering
%   \includegraphics[width=2.2 in]{airplane5}
%   \\
%  \end{minipage}%
% \caption{An example of Catmull-Clark solid.}
%\end{figure*}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> TO.tex <==
\usepackage{cleveref}


\section{Multi-resolution spline topology optimization with tricubic approximation of Catmull-Clark volumes}
\label{sec:optimization}

In this section, we present a multi-resolution 3D  topology optimization framework based on isogeometric analysis with the proposed unstructured spline solid representation. 
The proposed topology optimization framework has the following advantages:
 
\begin{itemize}
\item The proposed framework can realized the seamless data integration of geometric modeling, physical simulation and topology optimization, which is currently a bottleneck problem in generative design;
\item The final topology optimization results have a spline representation, which can be imported to CAD applications directly;
\item The subdivision geometry representation naturally has a multi-resolution topology optimization scheme, by which the computational efficiency can be significantly improved for high-resolution design optimization.  
\end{itemize}


In the following, based on the proposed spline approximation of Catmull-Clark solid,  we firstly introduce the isogeometric analysis framework for linear elastic problems. Then the formulation of topology optimization and multi-resolution scheme are presented in details.

\subsection{Solving linear elasticity problems by IGA with tricubic spline approximation of Catmull-Clark volumes}
\label{sec:IGAsolving}

Linear elasticity problems can be described as: find $u_i: \bar{\Omega}\rightarrow R$, such that
\begin{subequations}
\begin{align}
\sigma_{ij,j}+f_i&=0\quad \text{in} \Omega\\
u_i&=g_i\quad \text{on} \Gamma_{D_i} \\
\sigma_{ij}n_j&=h_i \quad\text{on} \Gamma_{N_i}
\end{align}
\end{subequations}
where $f_i:\Omega\rightarrow R$, $g_i:\Gamma_{D_i}\rightarrow R$, $h_i:\Gamma_{N_i}\rightarrow R$, and $i=1,2,3$ for 3-dimensional problem. The stress tensor $\bm{\sigma}=[\sigma_{ij}]$ is related to strain tensor as follows 
\begin{equation}\label{eq:stresstensor}\bm{\epsilon}=[\epsilon_{ij}],\quad \epsilon_{ij}=\frac{\frac{\partial u_i}{\partial x_j}+\frac{\partial u_j}{\partial x_i}}{2}\end{equation} . 

With matrix representation, the relation can be stated as
\[
\bm{\sigma}=\mathbf{D}\bm{\epsilon(\bm{u})}, 
\]
where
\[\mathbf{D}=\begin{bmatrix} \lambda+2\mu & \lambda & \lambda &0 & 0 &0 \\
\lambda & \lambda+2\mu & \lambda & 0 & 0 & 0 \\
\lambda & \lambda & \lambda+2\mu & 0 & 0 & 0 \\
0 & 0 & 0 & \mu & 0 & 0 \\
0 & 0 & 0 & 0 & \mu & 0 \\
0 & 0 & 0 & 0 & 0 & \mu \end{bmatrix},\]
and $\lambda, \mu$ are expressed with Young's modulus $E$ and Poisson's ratio $\nu$ as 
$$\lambda = \frac{\nu E}{(1+\nu)(1-2\nu)},\quad \mu = \frac{E}{2(1+\nu)}.$$

The weak form of elasticity problem is to find $\bm{u}$ from trial solution space $\bm{\mathcal{S}}=\{\bm{u}|u_i\in S_i \ \text{satisty}\ u_i=g_i \ \text{on} \ \Gamma_{D_i}\}$, and for all $\bm{\omega}$ from weighting space $\bm{\mathcal{V}}=\{\bm{\omega}|\omega_i\in \mathcal{V}_i\ \text{satisty}\ \omega_i=0 \ \text{on}\ \Gamma_{D_i}\}$, \[a(\bm{w},\bm{u})=L(\bm{w}),\]
where \begin{subequations}\label{eq:weakform}\begin{align}a(\bm{w},\bm{u})&=\int_{\Omega}\bm{\epsilon(\bm{w})}^T\mathbf{D}\bm{\epsilon(\bm{u})}d\Omega,\\
L(\bm{w})&=\int_{\Omega}\omega_if_id\Omega+\sum_{i=1}^d\left(\int_{\Gamma_{N_i}}\omega_ih_id\Gamma\right),
\end{align}\end{subequations}

In IGA, finite subspaces $\bm{\mathcal{S}^h}\subset \bm{\mathcal{S}}$ and $\bm{\mathcal{V}^h}\subset\bm{\mathcal{V}}$ are defined by the unstructured spline approximation of Catmull-Clark subdivision solid, which is also used to represent the geometry.  Hence the numerical solution $\bm{u}^h$ and test function $\bm{\omega}^h$ can be represented as linear combination of spline basis functions,
\begin{equation}\label{eq:NumSolRep}\begin{aligned}\bm{u}^h(\bm{x})&=\sum_{n=1}^{N_S} \bm{u}_n^hN_n(\bm{x}),\\
\bm{\omega}^h(\bm{x})&=\sum_{n=1}^{N_V} \bm{\omega}_n^hN_n(\bm{x}).
\end{aligned}\end{equation}
where $\bm{u}_n^h=[u_{n,x}^h,u_{n,y}^h,u_{n,z}^h]^T$ and $\bm{\omega}_n^h=[\omega_{n,x}^h,\omega_{n,y}^h,\omega_{n,z}^h]^T$ are coefficient vectors of $\bm{u^h}$ and $\bm{\omega^h}$, $N_S$ and $N_V$ represent the number of bases in space $\bm{\mathcal{S}}^h$ and $\bm{\mathcal{V}}^h$. By substituting Eq.(\ref{eq:NumSolRep}) into Eq. (\ref{eq:weakform}), a linear system can be derived as
\begin{equation}\label{eq:LinearEq}
\mathbf{K}\mathbf{U}=\mathbf{F}
\end{equation}
where the stiffness matrix $\mathbf{K}=\int_{\Omega}\mathbf{B}^T\mathbf{D}\mathbf{B}d\Omega$,  and \[\mathbf{B}=[\mathbf{B}_1,\mathbf{B}_2,\cdots,\mathbf{B}_n].\]
And for each shape function $N_i$, we have
\[\mathbf{B}_i=\begin{bmatrix}N_{i,x} & 0 & 0\\ 0 & N_{i,y} & 0\\
0 & 0 & N_{i,z}\\ 0 & N_{i,z} & N_{i,y} \\ N_{i,z} & 0 & N_{i,x}\\ N_{i,y} & N_{i,x} & 0\end{bmatrix}.\]

Once the displacements $\mathbf{U}$ are obtained by solving the linear system (\ref{eq:LinearEq}) with the given boundary conditions, the stress $\bm{\epsilon}$ on the geometric shape can be obtained by calculating the displacement gradient as in Eq. (\ref{eq:stresstensor}). 


\subsection{Isogeometric topology optimization framework with tricubic approximation of Catmull-Clark subdivision volumes }

Topology optimization distributes material in an optimal way, which maximize the stiffness of structure with the prescribed volume constraint. It is considered to minimize the compliance $c(\rho,u)$ under the volume constraint for the aim of topology optimization. In the discrete form, the compliance is expressed as\cite{X-Huang}
$$c(\rho)=\frac{1}{2} \mathbf{U}^T\mathbf{K}(\rho)\mathbf{U}, $$
which is the total strain energy of the system, where $\rho$ represents density variable, and $\mathbf{K}$ is the global stiffness matrix
\[\mathbf{K}=\int_{\Omega}\mathbf{B}^T\mathbf{D}(\rho)\mathbf{B}d\Omega,\]
The constitutive matrix $\mathbf{D}(\rho)$ depends on the material density, for 3-dimensional stress,  it can be expressed in terms of the
Young's modulus $E$ and Poisson's ratio, $\nu$ as follows
\[\mathbf{D}(\rho)=\frac{E(\rho)}{(1+\nu)(1-2\nu)}\begin{bmatrix} 1-\nu & \nu & \nu & 0 & 0 & 0\\
\nu & 1-\nu & \nu & 0 & 0 & 0\\
\nu & \nu & 1-\nu & 0 & 0 & 0\\
0 & 0 & 0 & \frac{1-2\nu}{2} & 0 & 0\\
0 & 0 & 0 & 0 & \frac{1-2\nu}{2} & 0 \\
0 & 0 & 0 & 0 & 0 & \frac{1-2\nu}{2}
\end{bmatrix}.\]
Then, the topology optimization problem can be stated as
\begin{subequations}\label{eq:TOP}
\begin{align}
minimize:\ &c(\rho)\ =\ \frac{1}{2}\mathbf{U}^T\mathbf{K}(\rho)\mathbf{U}\\
s.t : \ &\mathbf{K}(\rho)\mathbf{U}\ =\ \mathbf{F}\\
&\sum_{i=1}^N \rho_i V_i\ \leq\ V^*\\
&\rho_i\ = \ \rho_{min}\ or\ 1
\end{align}
\end{subequations}
where $\mathbf{U}$ is the global displacement vector. $V_i$ is the volume of an individual \Bezier block and $V^*$ is the target volume. The binary design variable $\rho_i$ denotes the density of $i$th \Bezier element. To avoid singularities of the global stiffness matrix $\mathbf{K}$, $\rho_{min}$ is set to be $0.0001$ .

In our framework, the geometry to be optimized is represented with multi-patch Bezier volumes. 
Suppose that the geometry $\Omega$ is composed of \Bezier blocks $\Omega_e, e=1,\cdots,N$. We solve the  displacements on these $\Omega_e$ by multi-block IGA method described in subsection \ref{sec:IGAsolving} . In this paper, Poisson's ratio is assumed to be independent of the density and Young's modulus is dependent of the variable density, the Young's modulus and constitutive matrix can be expressed using the following equations:
\begin{equation*}
E(\rho_e)\ =\ (\mu_{min}+(1-\mu_{min})\ \rho_e^p\ )\ E^0
\end{equation*}
\begin{equation*}
\mathbf{D}(\rho_e)\ =\ (\mu_{min}+(1-\mu_{min})\ \rho_e^p\ )\ \mathbf{D}^0
\end{equation*}
where $p$ is a penalization parameter (typically $p = 3$) and $E^0$ is the Young's modulus for solid material and $\mu_{min}$ is a minimum fraction of $E^0$ imposed to ensure that numerical difficulties due to $0$ densities are avoided, and $\mu_{min}$ is set to be  $10^{-9}-10^{-7}$. This leads to the following expression for the global stiffness matrix:
\begin{equation}
\mathbf{K}(\rho)\ =\ \sum_{e=1}^N\mathbf{K}_e\ =\ \sum_{e=1}^N(\mu_{min}+(1-\mu_{min})\ \rho_e^p\ )\ \mathbf{K}_e^0
\end{equation}
where the summation sign implies finite element summation over all the elements and $\mathbf{K}_e^0$ is the local stiffness matrix for element $e$ with Young's modulus $E^0$.

 


Once the displacement vector $\mathbf{U}$ for the current geometry is computed via solving the linear system (\ref{eq:TOP}b), we evaluate the objective function (\ref{eq:TOP}a) under the constraint (\ref{eq:TOP}c). Therefore, the derivatives of the total strain energy $c$ with respect to the design variable $\rho_e^i$ can be computed as
\begin{equation}
\frac{\partial c}{\partial \rho_e}\ =\ -\frac{p}{2}(\rho_e)^{p-1}\mathbf{u}_e^T(K_e)^0\mathbf{u}_e
\end{equation}

Then the sensitivity of density element $e$ can be computed as
\begin{equation*}
\alpha_e\ =\ -\frac{\partial c}{\partial \rho_e}
\end{equation*}
A large value of sensitivity indicates that the the current element has a high impact on the change of the strain energy.

\subsection{Multi-resolution topology optimization scheme with tricubic approximation of Catmull-Clark subdivision volumes }

In general topology optimization framework, the number of design variables has to be very large to obtain a high-resolution design, which will cause an efficiency problem of solving a large linear system for  physical simulation in each iteration step. The proposed trivariate spline model has a natural multi-resolution property, that is, for a specified shape, we can use a hierarchical volume parameterization  $\mathbf{T}_i(u,v,w)$ ($i=0,1,2,\cdots, N$) with different number of \Bezier blocks to represent the same geometry. 
In order to improve the efficiency of the optimization procedure, for each iteration, we solve the equilibrium equation of linear elasticity problem  on a volume parameterization $\mathbf{T}_i(u,v,w)$ with a fixed resolution to obtain a numerical solution with approximation error, which is smaller than a given tolerance. Then the density and sensitivity on the volume parameterization $\mathbf{T}_{j(u,v},w)$ ($j=i+1, i+2, \cdots, N$) with higher-resolution can be exactly computed from the isogeometric solution on $\mathbf{T}_i(u,v,w)$. Thanks to this multi-resolution scheme, we can efficiently achieve topology optimization  with high-resolution design, which can be produce more details in the optimization results. 

The proposed multi-resolution topology optimization problem can be described as follows:
\begin{subequations}\label{eq:MTOP}
\begin{align}
minimize:\ &c(\rho)\ =\ \frac{1}{2}\sum_{e=1}^N(\mathbf{u}^e)^T\mathbf{K_e}(\rho)\mathbf{u}^e=\frac{1}{2}\sum_{e=1}^N\sum_{i=1}^{N^e}(\mathbf{u}^e)^T\mathbf{K_e^i}(\rho)\mathbf{u}^e\\
s.t : \ &\sum_{e=1}^N\sum_{i=1}^{N^e}\mathbf{K_e^i}(\rho)\mathbf{U}\ =\ \mathbf{F}\\
&\sum_{e=1}^N\sum_{i=1}^{N^e} V_e^i\rho_e^i\ \leq\ V^*\\
&\rho_e^i\ = \ \rho_{min}\ or\ 1
\end{align}
\end{subequations}
where $N$ is number of \Bezier blocks in the volume parameterization $\mathbf{T}_i(u,v,w)=\bigcup_{e=1}^N\Omega_e$  , by which the displacement $\mathbf{u}$ is approximated. In the subdivision procedure, each \Bezier block $\Omega_e$ is divided into eight \Bezier sub-blocks $\Omega_e^i, i=1,\cdots,8$. The density variables $\rho_e^i$ are defined on the finer mesh $\bigcup_{e=1,i=1}^{N,N_e}\Omega_e^i$,  in which  $N^e=2^{3n}$, with $n$ is subdivision times from the fixed volume parameterization  $\mathbf{T}_i(u,v,w)=\bigcup_{e=1}^N\Omega_e$. 

 
The local stiffness matrix on each block in the volume parameterization $\mathbf{T}_{j}(u,v,w)$ ($j=i+1, i+2, \cdots, N$) with higher-resolution can be computed in the parametric domain as
\[K_e^i=\int_{\Omega_e^i}\mathbf{B}^T\mathbf{D}(\rho)\mathbf{B}d\Omega_e=\int_0^1\int_0^1\int_0^1 \mathbf{B}^T\mathbf{D}(\rho_e)\mathbf{B}J_e^id\xi d\eta d\zeta\]
where $\mathbf{B}$ is strain-displacement matrix of shape function defined on coarser mesh $\Omega_e$, and $J_e^i$ is Jacobian of mapping from unit cube to density element $\Omega_e^i$. Therefore, in our mutli-resolution framework, we solve the linear elasticity problems on a fixed volume parameterization  $\mathbf{T}_i(u,v,w)$ in each iteration, and compute the sensitivity   of the following volume parameterization $\mathbf{T}_{j}(u,v,w)$ ($j=i+1, i+2, \cdots, N$) with high-resolution directly and explicitly. This procedure can be proceeded without projection used in ~\cite{MTOP} and without any more complex computation used in~\cite{MTOPIGA}, which is very easy to be implemented.

The derivatives of the total strain energy $c$ with respect to the design variable $\rho_e^i$ can be computed as
\begin{equation}
\frac{\partial c}{\partial \rho_e^i}\ =\ -\frac{p}{2}(\rho_e)^{p-1}\mathbf{u}_e^T(K_e^i)^0\mathbf{u}_e, 
\end{equation}
and the sensitivity of $e^i$ can be computed as follows, 
\begin{equation*}
\alpha_e^i\ =\ -\frac{\partial c}{\partial \rho_e^i}.
\end{equation*}


%Figure ? shows the displacement defined on the coarse mesh $M_c$, while the density variables are defined on finer mesh $M_f$, where the elements of finer mesh $M_f$ are subdivision solids of element of coarse mesh $M_c$.

%\subsection{Filter scheme}

%To avoid numerical instabilities such as checkerboard and mesh-dependency, the filter technique is applied to smooth the sensitivities in the whole design domain. 


%In this paper, we modify the sensitivity of the original $i$th element by combining the sensitivities of the $i$th element with its adjacent element and recalculating by a set of weight. It is equivalent to we make a spherical range $\Omega_i$ with the center of the $i$th element as the center and a radius $r$ as the spherical range (a figre to show this). The sensitivity of the $i$th element is combined with that of all the elements in this range. The modified sensitivity is
%\begin{equation}
%\hat{\alpha_i}\ =\ \frac{\sum \limits_{i=1}^n\omega_{ij}\alpha_j}{\sum \limits_{i=1}^n\omega_{ij}}
%\end{equation}
%where n is the total number of elements in the domain $\Omega_i$, $\omega_{ij}$ is weight factor given as
%\begin{equation*}
%\omega_{ij}\ =\ r-r_{ij}
%\end{equation*}
%where $r_{ij}$ denotes the distance between the center of the element i and element j. In this paper, we set
%\begin{equation*}
%r\ =\ 2\frac{1}{n}\sum_{j=1}^nr_{ij}
%\end{equation*}
%where $n$ denotes the number of adjacent elements of $i$th element. (If $i$th element is a internal hexahedral mesh, then $n=6$).
%\par
%According to BESO algorithm, it is hard to convergent with above sensitivity numbers. Computational experience has shown that averaging the sensitivity number with its historical information is an effective way to avoid this problem. So the final sensitivity of the $i$th element is
%\begin{equation}
%\tilde{\alpha}_i\ =\ %\frac{1}{2}(\hat{\alpha_{i,k}}+\hat{\alpha_{i,k+1}})
%\end{equation}
%where $k$ is the current iteration number, then let $\hat{\alpha_{i,k}}\ =\ \tilde{\alpha}_i$. Therefore, the modified sensitivity of $i$th element considers the information of the sensitivity of its neighbors and historical iterations, avoids numerical instability effectively.


%\subsection{The procedure of topology optimization using Catmull-Clark subdivision solids}
%Since the Catmull-Clark subdivision limit solids of a model is the same as the Catmull-Clark subdivision limit solids of the model that subdivided by Catmull-Clark subdivision, we can optimize the topology of a rough model's Catmull-Clark subdivision limit solids, that is, an approximate B\'ezier solid. The specific steps of topology optimization are:
%\begin{enumerate}
%    \item Input a rough hexahedral mesh model $M$ and set the density $\rho$ of each cell to $1$.
%    \item Define the BESO parameter such as objective volume $V^*$, evolutionary ratio $ER$ and penalty exponent $p$.
%    \item Use the Catmull-Clark subdivision secheme to subdivide $M$ to the appropriate extent. The sensitivity of the subdivided elements inherits the sensitivity of the previous level. Then construct the control mesh of B\'ezier solid for each element by the method of section 4.
%    \item Perform finite element analysis, i.e. construct the stiffness matrix $K$ and the right end term $f$.
%    \item Calculate the displacement $u$ by Eq.2, and perform sensitivity analysis by Eq.10, then filter each element by Eq.11, Eq.12.
%    \item Determine the volume $V_i$ to be retained by $ER$ for the current iteration
%    \begin{equation*}
%    V_i\ =\ V_{i-1}(1-ER)
%    \end{equation*}
%    \item  Sort all elements by sensitivity from small to large. The density $\rho$ of the $n$ elements that need to be deleted from the beginning is set to $\rho_{min}$ and the density $\rho$ of the remaining elements remains unchanged. Record the density to calculate the stiffness matrix by Eq.5 for the next iteration.
%    \item Repeat 4-7 until the objective volume is achieved i.e. $V_i\ =\ V^*$. Then delete the element whose $\rho\ =\ \rho_{min}$.
%\end{enumerate}
%
%
%In our framework, isogeometric analysis is employed for numerical simulation, and the final topology optimization geometry is a set of cubic patches with $C^2$/$C^0$ contiunity, which can be imported for CAD applications directly.

%[MTOP] Tam H. Nguyen, Glaucio H. Paulino, Junho Song, Chau H. Le, A computational paradigm for multiresolution topology optimization (MTOP), Struc Multidisc Optim, 41: 525-539, 2010.



\subsection{The procedure of topology optimization using Catmull-Clark subdivision solids}


Since the Catmull-Clark subdivision limit solids of a model is the same as the Catmull-Clark subdivision limit solids of the model that subdivided by Catmull-Clark subdivision, we can optimize the topology of a rough model's Catmull-Clark subdivision limit solids, that is, an approximate B\'ezier solid. The specific steps of topology optimization are:
\begin{enumerate}
    \item Input a rough hexahedral mesh model $M$ and set the density $\rho$ of each cell to $1$.
    \item Define the BESO parameter such as objective volume $V^*$, evolutionary ratio $ER$ and penalty exponent $p$.
    \item Use the Catmull-Clark subdivision scheme to subdivide $M$ to the appropriate extent. The density of the subdivided elements inherits the sensitivity of the previous level. Then construct the control lattice of B\'ezier solid for each element by the method of section 4.
    \item Perform finite element analysis, i.e. construct the stiffness matrix $K$ and the right end term $f$.
    \item Calculate the displacement $u$ by Eq.15(b), and perform sensitivity analysis for next level subdivision mesh by Eq.16. %then filter each element by Eq.11, Eq.12.
    \item Determine the volume $V_i$ to be retained by $ER$ for the current iteration
    \begin{equation*}
    V_i\ =\ V_{i-1}(1-ER)
    \end{equation*}
    \item  Sort all elements by sensitivity from small to large. The density $\rho$ of the $n$ elements that need to be deleted from the beginning is set to $\rho_{min}$ and the density $\rho$ of the remaining elements remains unchanged. Record the density to calculate the stiffness matrix by Eq.13 for the next iteration.
    \item Repeat 4-7 until the objective volume is achieved i.e. $V_i\ =\ V^*$. Then delete the element whose $\rho\ =\ \rho_{min}$.
\end{enumerate}



==> VolumeConstruction.tex <==

\begin{figure}[htb]
 \begin{minipage}[c]{0.4\textwidth}
    \centering
    \includegraphics[width=1.8 in]{datpoint1}
 \\   (a)
 \end{minipage}\\
 \begin{minipage}[c]{0.4\textwidth}
   \centering
   \includegraphics[width=1.8 in]{datpoint2}
   \\ (b)
  \end{minipage}\\
 \caption{A hexahedral element (a) and its corresponding 64 B\'ezier control points (b). The red, blue, yellow and green dots represent cell points, face points, edge points and corner points, respectively.}
\end{figure}\label{fig:control}

\begin{figure*}[htb]
\begin{minipage}[c]{0.25\textwidth}
    \centering
    \includegraphics[width=1.3 in]{intermask.eps}
 \\   (a)
 \end{minipage}%
 \begin{minipage}[c]{0.25\textwidth}
   \centering
   \includegraphics[width=1.8 in]{edgemask.eps}
  \\ (b)
  \end{minipage}%
\begin{minipage}[c]{0.25\textwidth}
    \centering
  \includegraphics[width=1.3 in]{facemask.eps}
 \\ (c)
 \end{minipage}%
  \begin{minipage}[c]{0.25\textwidth}
   \centering
  \includegraphics[width=1.7in, height=2.0in]{cornermask.pdf}
   \\ (d)
  \end{minipage}\\
 \caption{Generalized masks for interior, edge, face and corner points.}
\end{figure*}\label{fig:generalizedmask}


\begin{figure*}[htb]
\begin{minipage}[c]{0.25\textwidth}
    \centering
    \includegraphics[width=1.45 in]{interiorpoint.eps}
 \\   (a)
 \end{minipage}%
 \begin{minipage}[c]{0.25\textwidth}
   \centering
   \includegraphics[width=1.45 in]{edgepoint.eps}
  \\ (b)
  \end{minipage}%
\begin{minipage}[c]{0.25\textwidth}
    \centering
  \includegraphics[width=1 in]{facepoint.eps}
 \\ (c)
 \end{minipage}%
  \begin{minipage}[c]{0.25\textwidth}
   \centering
  \includegraphics[width=1.7in]{cornerpoint.eps}
   \\ (d)
  \end{minipage}\\
 \caption{Masks for interior, edge, face and corner points in regular.}
\end{figure*}\label{fig:regularmask}


\begin{figure*}[htb]
\begin{minipage}[c]{0.19\textwidth}
    \centering
    \includegraphics[width=1.2 in]{testmesh}
 \\   (a) Input hex-mesh with singularity
 \end{minipage}%
 \begin{minipage}[c]{0.19\textwidth}
    \centering
    \includegraphics[width=1.2 in]{testmesh2}
 \\   (b) Our construction
 \end{minipage}%
 \begin{minipage}[c]{0.19\textwidth}
   \centering
   \includegraphics[width=1.2 in]{testmesh3}
   \\ (c) Interior view of (b)
  \end{minipage}%
 \begin{minipage}[c]{0.19\textwidth}
    \centering
    \includegraphics[width=1.2 in]{comparetestmesh1}
 \\   (d) Approximation error
 \end{minipage}%
 \begin{minipage}[c]{0.22\textwidth}
   \centering
   \includegraphics[width=1.3 in]{comparetestmesh2}
   \\ (e) Interior view of (d)
  \end{minipage}%
\begin{minipage}[c]{0.05\textwidth}
    \centering
  \includegraphics[width=0.2 in]{compare7mesh4}
 \\
 \end{minipage}\\
 \caption{A simple example.}
\end{figure*}


\begin{figure*}[htb]
\begin{minipage}[c]{0.19\textwidth}
    \centering
    \includegraphics[width=1.35 in]{ex8a}
 \\   (a)
 \end{minipage}%
 \begin{minipage}[c]{0.19\textwidth}
   \centering
   \includegraphics[width=1.4 in]{1ex8c}
   \\ (b)
  \end{minipage}%
\begin{minipage}[c]{0.19\textwidth}
    \centering
  \includegraphics[width=1.25 in]{1ex8d}
 \\ (c)
 \end{minipage}%
 \begin{minipage}[c]{0.19\textwidth}
    \centering
  \includegraphics[width=1.4 in]{1ex8error}
 \\ (d)
 \end{minipage}%
 \begin{minipage}[c]{0.19\textwidth}
    \centering
  \includegraphics[width=0.95 in]{1ex8error1}
 \\ (e)
 \end{minipage}%
 \begin{minipage}[c]{0.05\textwidth}
    \centering
  \includegraphics[width=0.23 in]{cuperror}
 \\ 
 \end{minipage}\\
 \caption{Cup.}
\end{figure*}

\begin{figure*}[htb]
\begin{minipage}[c]{0.2\textwidth}
    \centering
    \includegraphics[width=1.4 in]{ex5a}
 \\   (a)
 \end{minipage}%
 \begin{minipage}[c]{0.2\textwidth}
   \centering
   \includegraphics[width=1.4 in]{1ex5c}
   \\ (b)
  \end{minipage}%
\begin{minipage}[c]{0.2\textwidth}
    \centering
  \includegraphics[width=1.1 in]{1ex5d}
 \\ (c)
 \end{minipage}%
 \begin{minipage}[c]{0.2\textwidth}
    \centering
  \includegraphics[width=1.4 in]{1ex5error}
 \\ (d)
 \end{minipage}%
 \begin{minipage}[c]{0.2\textwidth}
    \centering
  \includegraphics[width=0.85 in]{1ex5error1}
 \\ (e)
 \end{minipage}%
  \begin{minipage}[c]{0.05\textwidth}
    \centering
  \includegraphics[width=0.2 in]{horseerror}
 \\
 \end{minipage}\\
 \caption{Horse.}
\end{figure*}




\begin{figure*}[htb]
\begin{minipage}[c]{0.2\textwidth}
    \centering
    \includegraphics[width=1.15 in]{ex6a}
 \\   (a)
 \end{minipage}%
 \begin{minipage}[c]{0.2\textwidth}
   \centering
   \includegraphics[width=1.15 in]{1ex6c}
   \\ (b)
  \end{minipage}%
\begin{minipage}[c]{0.2\textwidth}
    \centering
  \includegraphics[width=0.9 in]{1ex6d}
 \\ (c)
 \end{minipage}%
 \begin{minipage}[c]{0.2\textwidth}
    \centering
  \includegraphics[width=1.15 in]{1ex6error}
 \\ (d)
 \end{minipage}%
 \begin{minipage}[c]{0.2\textwidth}
    \centering
  \includegraphics[width=0.8 in]{1ex6error1.png}
 \\ (e)
 \end{minipage}%
  \begin{minipage}[c]{0.05\textwidth}
    \centering
  \includegraphics[width=0.23 in]{handerror1}
 \\
 \end{minipage}\\
 \caption{Hand.}
\end{figure*}


\section{Constructing the approximation of Catmull-Clark subdivision solids with tricubic volumes}
\label{sec:approx}


Volumetric spline modeling of complex geometry is a key issue for isogeometric analysis. In this section, based on the proposed limit point formula, we will present a volumetric spline modeling method from an input hex-mesh, which leads to an approximation of Catmull-Clark subdivision solid  with a minimal set of tricubic spline volumes.

The corresponding problem can be described as follows: for each cell of a given hexahedral mesh $H$, construct a control lattice such that the corresponding B\'ezier volume is an approximation of the limit Catmull-Clark subdivision volume generated from $H$.

Given an hexahedral element $M$ and its corresponding control lattice is denoted as  $M'$. The $64$ B\'ezier control points are calculated from the vertices of $M$ and its one-neighbouring hexahedral elements. The eight local vertices in an hexahedral element are shown in Fig. \ref{fig:control}(a), and corresponding B\'ezier control points are shown with different colors in Fig. \ref{fig:control}(b). Note that the hexahedron in Fig. \ref{fig:control} are used only to visualize these B\'ezier control points, rather than being an actual refinement of the hexahedral element.

To generate a spline volume approximating the Catmull-Clark limit solid, a basic requirement is that the generated spline volume should  interpolate the limit point of the Catmull-Clark subdivision solid obtained from the input hex-mesh. To achieve this goal, we need to make the eight corner control points of the control lattice generated in the first step equal to the limit point of the Catmull-Clark subdivision solid. And obviously, the Catmull-Clark limit solid of a mesh is the same as the Catmull-Clark limit solid after it is subdivided once. So we assume that the current mesh is a mesh after a certain mesh is subdivided. So according to the limit point formula of Catmull-Clark
subdivision volume, we set the mask of each point of the control lattice in Fig.5.

Referring to Fig.5, mask (a) is used (in eight orientations) to
create the eight red interior points in Fig.4(b), corresponding to a interior point near each corner point; mask (b) is used to create the yellow edge points in Fig.4(b), corresponding to a edge point near the corner point in the edge; mask (c) is used to create the blue face points in Fig.4(b), corresponding to a face point near the corner point in the face; finally, mask (d) is used to create the green corner
points, corresponding to each corner point of the hex-mesh. Note that there has a characteristic that the face points, edge points, and corner points are the average of interior point of all adjacent cells, so you can simply calculate the interior points of all elements, and then calculate other edges, face and cell points based on these interior points. And when there has no singular case, masks for interior, edge, face and corner points in regular case are shown in Fig.6.

 
 %For the case of hex-element without extraordinary vertices, according to the property of cubic B-spline volumes, we can construct the interior control points(red), edge control points(yellow), face control points(blue), corner control points(green) according to the masks shown in Fig. \ref{fig:regularmask}.

 %For the case of hex-element with extraordinary vertices, according to the we st pointet thula (\ref{eqn:limit}), el formimi mask of the interior point as shown in Fig. \ref{fig:sigmask} (d), where $n$ is the degree of the point corresponding to the interior point, $m$ is the valence of one adjacent edge of the point.

 




%Some modeling examples are shown in Fig.6, Fig. 7, Fig.8, Fig.9 and Fig.10, in which (a) is the input hex-mesh, (b) and (c) are the tricubic spline volume approximation from different view, (e) and (f) are the colormap of the approximation from different view.  







